Decomposing Magnetic Fields in Three Dimensions over the Central Molecular Zone

Measuring magnetic fields in the interstellar medium and obtaining their distribution along line-of-sight is very challenging with the traditional techniques. The Velocity Gradient Technique (VGT), which utilizes anisotropy of magnetohydrodynamic (MHD) turbulence, provides an attractive solution. Targeting the central molecular zone (CMZ), we test this approach by applying the VGT to $\rm ^{12}CO$ and $\rm ^{13}CO$ (J = 1-0) data cubes. We first used the SCOUSEPY algorithm to decompose the CO line emissions into separate velocity components, and then we constructed pseudo-Stokes parameters via the VGT to map the plane-of-the-sky magnetic fields in three-dimension. We present the decomposed magnetic field maps and investigate their significance. While the line-of-sight integrated magnetic field orientation is shown to be consistent with the polarized dust emission from the Planck survey at 353 GHz, individual velocity components may exhibit different magnetic fields. We present a scheme of magnetic field configuration in the CMZ based on the decomposed magnetic fields. In particular, we observe a nearly vertical magnetic field orientation in the dense clump near the Sgr B2 and a change in the outflow regions around the Sgr A*. Two high-velocity structures associated with an expanding ring in the CMZ show distinct swirling magnetic field structures. These results demonstrate the potential power of the VGT to decompose velocity or density-dependent magnetic structures.

==> example <==
@ARTICLE{2015A&A...576A.105P,
       author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and {Alina}, D. and {Alves}, M.~I.~R. and {Aniano}, G. and {Armitage-Caplan}, C. and {Arnaud}, M. and {Arzoumanian}, D. and {Ashdown}, M. and {Atrio-Barandela}, F. and {Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Battaner}, E. and {Benabed}, K. and {Benoit-L{\'e}vy}, A. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bracco}, A. and {Burigana}, C. and {Cardoso}, J. -F. and {Catalano}, A. and {Chamballu}, A. and {Chiang}, H.~C. and {Christensen}, P.~R. and {Colombi}, S. and {Colombo}, L.~P.~L. and {Combet}, C. and {Couchot}, F. and {Coulais}, A. and {Crill}, B.~P. and {Curto}, A. and {Cuttaia}, F. and {Danese}, L. and {Davies}, R.~D. and {Davis}, R.~J. and {de Bernardis}, P. and {de Rosa}, A. and {de Zotti}, G. and {Delabrouille}, J. and {Dickinson}, C. and {Diego}, J.~M. and {Donzelli}, S. and {Dor{\'e}}, O. and {Douspis}, M. and {Dupac}, X. and {Efstathiou}, G. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Falgarone}, E. and {Fanciullo}, L. and {Ferri{\`e}re}, K. and {Finelli}, F. and {Forni}, O. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Galeotta}, S. and {Ganga}, K. and {Ghosh}, T. and {Giard}, M. and {Giraud-H{\'e}raud}, Y. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gregorio}, A. and {Gruppuso}, A. and {Guillet}, V. and {Hansen}, F.~K. and {Harrison}, D.~L. and {Helou}, G. and {Hern{\'a}ndez-Monteagudo}, C. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Hobson}, M. and {Holmes}, W.~A. and {Hornstrup}, A. and {Huffenberger}, K.~M. and {Jaffe}, A.~H. and {Jaffe}, T.~R. and {Jones}, W.~C. and {Juvela}, M. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kisner}, T.~S. and {Kneissl}, R. and {Knoche}, J. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lawrence}, C.~R. and {Leonardi}, R. and {Levrier}, F. and {Liguori}, M. and {Lilje}, P.~B. and {Linden-V{\o}rnle}, M. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maino}, D. and {Mandolesi}, N. and {Maris}, M. and {Marshall}, D.~J. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Matarrese}, S. and {Mazzotta}, P. and {Melchiorri}, A. and {Mendes}, L. and {Mennella}, A. and {Migliaccio}, M. and {Miville-Desch{\^e}nes}, M. -A. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Mortlock}, D. and {Munshi}, D. and {Murphy}, J.~A. and {Naselsky}, P. and {Nati}, F. and {Natoli}, P. and {Netterfield}, C.~B. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {Oxborrow}, C.~A. and {Pagano}, L. and {Pajot}, F. and {Paoletti}, D. and {Pasian}, F. and {Pelkonen}, V. -M. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Piacentini}, F. and {Piat}, M. and {Pietrobon}, D. and {Plaszczynski}, S. and {Pointecouteau}, E. and {Polenta}, G. and {Popa}, L. and {Pratt}, G.~W. and {Prunet}, S. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reinecke}, M. and {Remazeilles}, M. and {Renault}, C. and {Ricciardi}, S. and {Riller}, T. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rusholme}, B. and {Sandri}, M. and {Scott}, D. and {Soler}, J.~D. and {Spencer}, L.~D. and {Stolyarov}, V. and {Stompor}, R. and {Sudiwala}, R. and {Sutton}, D. and {Suur-Uski}, A. -S. and {Sygnet}, J. -F. and {Tauber}, J.~A. and {Terenzi}, L. and {Toffolatti}, L. and {Tomasi}, M. and {Tristram}, M. and {Tucci}, M. and {Umana}, G. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, B. and {Vielva}, P. and {Villa}, F. and {Wade}, L.~A. and {Wandelt}, B.~D. and {Zonca}, A.},
        title = "{Planck intermediate results. XX. Comparison of polarized thermal emission from Galactic dust with simulations of MHD turbulence}",
      journal = {\aap},
     keywords = {ISM: general, dust, extinction, ISM: magnetic fields, ISM:, clouds, infrared: ISM, submillimeter: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = apr,
       volume = {576},
          eid = {A105},
        pages = {A105},
          doi = {10.1051/0004-6361/201424086},
archivePrefix = {arXiv},
       eprint = {1405.0872},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...576A.105P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2016MNRAS.457.2675H,
       author = {{Henshaw}, J.~D. and {Longmore}, S.~N. and {Kruijssen}, J.~M.~D. and {Davies}, B. and {Bally}, J. and {Barnes}, A. and {Battersby}, C. and {Burton}, M. and {Cunningham}, M.~R. and {Dale}, J.~E. and {Ginsburg}, A. and {Immer}, K. and {Jones}, P.~A. and {Kendrew}, S. and {Mills}, E.~A.~C. and {Molinari}, S. and {Moore}, T.~J.~T. and {Ott}, J. and {Pillai}, T. and {Rathborne}, J. and {Schilke}, P. and {Schmiedeke}, A. and {Testi}, L. and {Walker}, D. and {Walsh}, A. and {Zhang}, Q.},
        title = "{Molecular gas kinematics within the central 250 pc of the Milky Way}",
      journal = {\mnras},
     keywords = {stars: formation, ISM: clouds, ISM: kinematics and dynamics, ISM: structure, Galaxy: centre, galaxies: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = apr,
       volume = {457},
       number = {3},
        pages = {2675-2702},
          doi = {10.1093/mnras/stw121},
archivePrefix = {arXiv},
       eprint = {1601.03732},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.457.2675H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999ARA&A..37...37K,
       author = {{Kulsrud}, Russell M.},
        title = "{A Critical Review of Galactic Dynamos}",
      journal = {\araa},
     keywords = {MHD DYNAMOS, GALACTIC MAGNETIC FIELDS, ALPHA EFFECT, FLUX EXPULSION, SMALL-SCALE FIELDS},
         year = 1999,
        month = jan,
       volume = {37},
        pages = {37-64},
          doi = {10.1146/annurev.astro.37.1.37},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ARA&A..37...37K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002ApJ...564..291C,
       author = {{Cho}, Jungyeon and {Lazarian}, Alex and {Vishniac}, Ethan T.},
        title = "{Simulations of Magnetohydrodynamic Turbulence in a Strongly Magnetized Medium}",
      journal = {\apj},
     keywords = {ISM: General, Methods: Numerical, Magnetohydrodynamics: MHD, Turbulence, Astrophysics},
         year = 2002,
        month = jan,
       volume = {564},
       number = {1},
        pages = {291-301},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...564..291C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992A&A...264..326L,
       author = {{Lazarian}, Alexander},
        title = "{Diffusion-generated electromotive force and seed magnetic field problem}",
      journal = {\aap},
     keywords = {Electromotive Forces, Galactic Evolution, Interstellar Magnetic Fields, Magnetic Diffusion, Computational Astrophysics, Cosmic Plasma, Interstellar Gas, Ionized Gases, Astrophysics},
         year = 1992,
        month = oct,
       volume = {264},
       number = {1},
        pages = {326-330},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992A&A...264..326L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1988ASSL..133.....R,
       author = {{Ruzmaikin}, Aleksandr A. and {Sokolov}, Dmitrii D. and {Shukurov}, Anvar M.},
        title = "{Magnetic Fields of Galaxies}",
         year = 1988,
       volume = {133},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988ASSL..133.....R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994PhRvL..72.1651G,
       author = {{Gruzinov}, A.~V. and {Diamond}, P.~H.},
        title = "{Self-consistent theory of mean-field electrodynamics}",
      journal = {\prl},
     keywords = {47.65.+a, 03.50.De, 91.25.Cw, Classical electromagnetism Maxwell equations, Origins and models of the magnetic field, dynamo theories},
         year = 1994,
        month = mar,
       volume = {72},
       number = {11},
        pages = {1651-1653},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994PhRvL..72.1651G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...550..752V,
       author = {{Vishniac}, Ethan T. and {Cho}, Jungyeon},
        title = "{Magnetic Helicity Conservation and Astrophysical Dynamos}",
      journal = {\apj},
     keywords = {ISM: Magnetic Fields, Magnetic Fields, Magnetohydrodynamics: MHD, Turbulence, Astrophysics, Physics - Plasma Physics},
         year = 2001,
        month = apr,
       volume = {550},
       number = {2},
        pages = {752-760},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...550..752V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2022arXiv220301508H,
       author = {{Hu}, Yue and {Federrath}, Christoph and {Xu}, Siyao and {Mathew}, Sajay Sunny},
        title = "{The Velocity Statistics of Turbulent Clouds in the Presence of Gravity, Magnetic fields, Radiation, and Outflow Feedback}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = mar,
          eid = {arXiv:2203.01508},
        pages = {arXiv:2203.01508},
archivePrefix = {arXiv},
       eprint = {2203.01508},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220301508H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2014ApJ...780..144V,
       author = {{Vishniac}, Ethan T. and {Shapovalov}, Dmitry},
        title = "{Properties of Magnetic Helicity Flux in Turbulent Dynamos}",
      journal = {\apj},
     keywords = {ISM: general, magnetic fields, magnetohydrodynamics: MHD, turbulence},
         year = 2014,
        month = jan,
       volume = {780},
       number = {2},
          eid = {144},
        pages = {144},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...780..144V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021MNRAS.503.1290S,
       author = {{Santos-Lima}, R. and {Guerrero}, G. and {de Gouveia Dal Pino}, E.~M. and {Lazarian}, A.},
        title = "{Diffusion of large-scale magnetic fields by reconnection in MHD turbulence}",
      journal = {\mnras},
     keywords = {magnetic fields, magnetic reconnection, MHD, turbulence, methods: numerical, stars: formation, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = may,
       volume = {503},
       number = {1},
        pages = {1290-1309},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.503.1290S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@INPROCEEDINGS{2015ASSL..407..311L,
       author = {{Lazarian}, Alex and {Eyink}, Gregory L. and {Vishniac}, Ethan T. and {Kowal}, Grzegorz},
        title = "{Magnetic Reconnection in Astrophysical Environments}",
     keywords = {Physics, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Physics - Plasma Physics, Physics - Space Physics},
    booktitle = {Magnetic Fields in Diffuse Media},
         year = 2015,
       editor = {{Lazarian}, Alexander and {de Gouveia Dal Pino}, Elisabete M. and {Melioli}, Claudio},
       series = {Astrophysics and Space Science Library},
       volume = {407},
        month = jan,
        pages = {311},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ASSL..407..311L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1971ApJ...163..255P,
       author = {{Parker}, E.~N.},
        title = "{The Generation of Magnetic Fields in Astrophysical Bodies. II. The Galactic Field}",
      journal = {\apj},
         year = 1971,
        month = jan,
       volume = {163},
        pages = {255},
          doi = {10.1086/150765},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1971ApJ...163..255P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...528..723C,
       author = {{Chandran}, Benjamin D.~G. and {Cowley}, Steve C. and {Morris}, Mark},
        title = "{Magnetic Flux Accumulation at the Galactic Center and Its Implications for the Strength of the Pregalactic Magnetic Field}",
      journal = {\apj},
     keywords = {DIFFUSION, GALAXY: CENTER, GALAXY: EVOLUTION, MAGNETOHYDRODYNAMICS: MHD, ISM: MAGNETIC FIELDS, TURBULENCE, Diffusion, Galaxy: Center, Galaxy: Evolution, Magnetohydrodynamics: MHD, ISM: Magnetic Fields, Turbulence},
         year = 2000,
        month = jan,
       volume = {528},
       number = {2},
        pages = {723-733},
          doi = {10.1086/308184},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...528..723C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1974PASJ...26..117K,
       author = {{Kaifu}, N. and {Iguchi}, T. and {Kato}, T.},
        title = "{Gaseous Structure in the Galactic Center Region}",
      journal = {PASJ},
         year = 1974,
        month = jan,
       volume = {26},
        pages = {117},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1974PASJ...26..117K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2016MNRAS.457.2675H,
       author = {{Henshaw}, J.~D. and {Longmore}, S.~N. and {Kruijssen}, J.~M.~D. and {Davies}, B. and {Bally}, J. and {Barnes}, A. and {Battersby}, C. and {Burton}, M. and {Cunningham}, M.~R. and {Dale}, J.~E. and {Ginsburg}, A. and {Immer}, K. and {Jones}, P.~A. and {Kendrew}, S. and {Mills}, E.~A.~C. and {Molinari}, S. and {Moore}, T.~J.~T. and {Ott}, J. and {Pillai}, T. and {Rathborne}, J. and {Schilke}, P. and {Schmiedeke}, A. and {Testi}, L. and {Walker}, D. and {Walsh}, A. and {Zhang}, Q.},
        title = "{Molecular gas kinematics within the central 250 pc of the Milky Way}",
      journal = {\mnras},
     keywords = {stars: formation, ISM: clouds, ISM: kinematics and dynamics, ISM: structure, Galaxy: centre, galaxies: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = apr,
       volume = {457},
       number = {3},
        pages = {2675-2702},
          doi = {10.1093/mnras/stw121},
archivePrefix = {arXiv},
       eprint = {1601.03732},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.457.2675H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2019MNRAS.485.2457H,
       author = {{Henshaw}, J.~D. and {Ginsburg}, A. and {Haworth}, T.~J. and {Longmore}, S.~N. and {Kruijssen}, J.~M.~D. and {Mills}, E.~A.~C. and {Sokolov}, V. and {Walker}, D.~L. and {Barnes}, A.~T. and {Contreras}, Y. and {Bally}, J. and {Battersby}, C. and {Beuther}, H. and {Butterfield}, N. and {Dale}, J.~E. and {Henning}, T. and {Jackson}, J.~M. and {Kauffmann}, J. and {Pillai}, T. and {Ragan}, S. and {Riener}, M. and {Zhang}, Q.},
        title = "{`The Brick' is not a brick: a comprehensive study of the structure and dynamics of the central molecular zone cloud G0.253+0.016}",
      journal = {\mnras},
     keywords = {turbulence, stars: formation, ISM: clouds, ISM: kinematics and dynamics, ISM: structure, galaxy: centre, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = may,
       volume = {485},
       number = {2},
        pages = {2457-2485},
          doi = {10.1093/mnras/stz471},
archivePrefix = {arXiv},
       eprint = {1902.02793},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.485.2457H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1972ApJ...175L.127S,
       author = {{Scoville}, N.~Z.},
        title = "{Kinematics of Molecular Clouds Near the Galactic Center}",
      journal = {ApJL},
         year = 1972,
        month = aug,
       volume = {175},
        pages = {L127},
          doi = {10.1086/181000},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1972ApJ...175L.127S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2019PASJ...71S..19T,
       author = {{Tokuyama}, Sekito and {Oka}, Tomoharu and {Takekawa}, Shunya and {Iwata}, Yuhei and {Tsujimoto}, Shiho and {Yamada}, Masaya and {Furusawa}, Maiko and {Nomura}, Mariko},
        title = "{High-resolution CO images of the Galactic central molecular zone}",
      journal = {PASJ},
     keywords = {Galaxy: center, Galaxy: kinematics and dynamics, ISM: molecules, surveys},
         year = 2019,
        month = dec,
       volume = {71},
          eid = {S19},
        pages = {S19},
          doi = {10.1093/pasj/psy150},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PASJ...71S..19T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2000ApJ...539..273C,
       author = {{Cho}, Jungyeon and {Vishniac}, Ethan T.},
        title = "{The Anisotropy of Magnetohydrodynamic Alfv{\'e}nic Turbulence}",
      journal = {\apj},
     keywords = {ISM: General, Magnetic Fields, Magnetohydrodynamics: MHD, Turbulence, Astrophysics},
         year = 2000,
        month = aug,
       volume = {539},
       number = {1},
        pages = {273-282},
          doi = {10.1086/309213},
archivePrefix = {arXiv},
       eprint = {astro-ph/0003403},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...539..273C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{GL17,
       author = {{Gonz{\'a}lez-Casanova}, Diego F. and {Lazarian}, A.},
        title = "{Velocity Gradients as a Tracer for Magnetic Fields}",
      journal = {\apj},
     keywords = {ISM: kinematics and dynamics, ISM: magnetic fields, magnetohydrodynamics: MHD, turbulence, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jan,
       volume = {835},
       number = {1},
          eid = {41},
        pages = {41},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...835...41G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020A&A...641A..12P,
       author = {{Planck Collaboration} and {Aghanim}, N. and {Akrami}, Y. and {Alves}, M.~I.~R. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Ballardini}, M. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and {Basak}, S. and {Benabed}, K. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bracco}, A. and {Bucher}, M. and {Burigana}, C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Carron}, J. and {Chary}, R. -R. and {Chiang}, H.~C. and {Colombo}, L.~P.~L. and {Combet}, C. and {Crill}, B.~P. and {Cuttaia}, F. and {de Bernardis}, P. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {Di Valentino}, E. and {Dickinson}, C. and {Diego}, J.~M. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dupac}, X. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Falgarone}, E. and {Fantaye}, Y. and {Fernandez-Cobos}, R. and {Ferri{\`e}re}, K. and {Finelli}, F. and {Forastieri}, F. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frolov}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {G{\'e}nova-Santos}, R.~T. and {Gerbino}, M. and {Ghosh}, T. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Green}, G. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Guillet}, V. and {Handley}, W. and {Hansen}, F.~K. and {Helou}, G. and {Herranz}, D. and {Hivon}, E. and {Huang}, Z. and {Jaffe}, A.~H. and {Jones}, W.~C. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kiiveri}, K. and {Kim}, J. and {Krachmalnicoff}, N. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Le Jeune}, M. and {Levrier}, F. and {Liguori}, M. and {Lilje}, P.~B. and {Lindholm}, V. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Ma}, Y. -Z. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Marcos-Caballero}, A. and {Maris}, M. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Matarrese}, S. and {Mauri}, N. and {McEwen}, J.~D. and {Melchiorri}, A. and {Mennella}, A. and {Migliaccio}, M. and {Miville-Desch{\^e}nes}, M. -A. and {Molinari}, D. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Moss}, A. and {Natoli}, P. and {Pagano}, L. and {Paoletti}, D. and {Patanchon}, G. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Polastri}, L. and {Polenta}, G. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reinecke}, M. and {Remazeilles}, M. and {Renzi}, A. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Ruiz-Granados}, B. and {Salvati}, L. and {Sandri}, M. and {Savelainen}, M. and {Scott}, D. and {Sirignano}, C. and {Sunyaev}, R. and {Suur-Uski}, A. -S. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Tenti}, M. and {Toffolatti}, L. and {Tomasi}, M. and {Trombetti}, T. and {Valiviita}, J. and {Vansyngel}, F. and {Van Tent}, B. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wandelt}, B.~D. and {Wehus}, I.~K. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck 2018 results. XII. Galactic astrophysics using polarized dust emission}",
      journal = {\aap},
     keywords = {polarization, magnetic fields, turbulence, dust, extinction, local insterstellar matter, submillimeter: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = sep,
       volume = {641},
          eid = {A12},
        pages = {A12},
          doi = {10.1051/0004-6361/201833885},
archivePrefix = {arXiv},
       eprint = {1807.06212},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...641A..12P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{YL17a,
       author = {{Yuen}, Ka Ho and {Lazarian}, A.},
        title = "{Tracing Interstellar Magnetic Field Using Velocity Gradient Technique: Application to Atomic Hydrogen Data}",
      journal = {\apjl},
     keywords = {ISM: general, ISM: magnetic fields, ISM: structure, magnetohydrodynamics: MHD, radio lines: ISM, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2017,
        month = mar,
       volume = {837},
       number = {2},
          eid = {L24},
        pages = {L24},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...837L..24Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995ApJ...443..209A,
       author = {{Armstrong}, J.~W. and {Rickett}, B.~J. and {Spangler}, S.~R.},
        title = "{Electron Density Power Spectrum in the Local Interstellar Medium}",
      journal = {\apj},
     keywords = {Electron Density Profiles, Interstellar Matter, Power Spectra, Scintillation, Astronomical Models, Plasma Turbulence, Pulsars, Radio Astronomy, Astrophysics, ISM: STRUCTURE, RADIO CONTINUUM: ISM, STARS: PULSARS: GENERAL, TURBULENCE},
         year = 1995,
        month = apr,
       volume = {443},
        pages = {209},
          doi = {10.1086/175515},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...443..209A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010ApJ...710..853C,
       author = {{Chepurnov}, A. and {Lazarian}, A.},
        title = "{Extending the Big Power Law in the Sky with Turbulence Spectra from Wisconsin H{\ensuremath{\alpha}} Mapper Data}",
      journal = {\apj},
     keywords = {ISM: lines and bands, methods: data analysis, techniques: spectroscopic, turbulence, Astrophysics - Galaxy Astrophysics},
         year = 2010,
        month = feb,
       volume = {710},
       number = {1},
        pages = {853-858},
          doi = {10.1088/0004-637X/710/1/853},
archivePrefix = {arXiv},
       eprint = {0905.4413},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...710..853C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019ApJ...874..171C,
       author = {{Clark}, S.~E. and {Peek}, J.~E.~G. and {Miville-Desch{\^e}nes}, M. -A.},
        title = "{The Physical Nature of Neutral Hydrogen Intensity Structure}",
      journal = {\apj},
     keywords = {dust, extinction, ISM: magnetic fields, ISM: structure, magnetic fields, radio lines: ISM, turbulence, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = apr,
       volume = {874},
       number = {2},
          eid = {171},
        pages = {171},
          doi = {10.3847/1538-4357/ab0b3b},
archivePrefix = {arXiv},
       eprint = {1902.01409},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...874..171C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021ApJ...910..161Y,
       author = {{Yuen}, Ka Ho and {Ho}, Ka Wai and {Lazarian}, Alex},
        title = "{Technique for Separating Velocity and Density Contributions in Spectroscopic Data and Its Application to Studying Turbulence and Magnetic Fields}",
      journal = {\apj},
     keywords = {Interstellar magnetic fields, Interstellar medium, Interstellar dynamics, Interstellar atomic gas, Interstellar filaments, 845, 847, 839, 833, 842, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Physics - Data Analysis, Statistics and Probability, Physics - Fluid Dynamics},
         year = 2021,
        month = apr,
       volume = {910},
       number = {2},
          eid = {161},
        pages = {161},
          doi = {10.3847/1538-4357/abe4d4},
archivePrefix = {arXiv},
       eprint = {2012.15776},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...910..161Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2000ApJ...537..720L,
       author = {{Lazarian}, A. and {Pogosyan}, D.},
        title = "{Velocity Modification of H I Power Spectrum}",
      journal = {\apj},
     keywords = {Galaxy: Structure, ISM: Kinematics and Dynamics, Radio Lines: ISM, Astrophysics},
         year = 2000,
        month = jul,
       volume = {537},
       number = {2},
        pages = {720-748},
          doi = {10.1086/309040},
archivePrefix = {arXiv},
       eprint = {astro-ph/9901241},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...537..720L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CMZ,
       author = {{Hu}, Yue and {Lazarian}, A. and {Wang}, Q. Daniel},
        title = "{Multiscale magnetic fields in the central molecular zone: inference from the gradient technique}",
      journal = {\mnras},
     keywords = {magnetic field, turbulence, ISM:general, ISM:magnetic field, Galaxy: centre, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = mar,
       volume = {511},
       number = {1},
        pages = {829-842},
          doi = {10.1093/mnras/stac159},
archivePrefix = {arXiv},
       eprint = {2105.03605},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.511..829H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{H2,
       author = {{Hu}, Yue and {Lazarian}, A. and {Bialy}, Shmuel},
        title = "{Study Turbulence and Probe Magnetic Fields Using the Gradient Technique: Application to H I-to-H$_{2}$ Transition Regions}",
      journal = {\apj},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, 847, 845, 839, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = dec,
       volume = {905},
       number = {2},
          eid = {129},
        pages = {129},
          doi = {10.3847/1538-4357/abc3c6},
archivePrefix = {arXiv},
       eprint = {2008.00387},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...905..129H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014MNRAS.440.3370K,
       author = {{Kruijssen}, J.~M. Diederik and {Longmore}, Steven N. and {Elmegreen}, Bruce G. and {Murray}, Norman and {Bally}, John and {Testi}, Leonardo and {Kennicutt}, Robert C.},
        title = "{What controls star formation in the central 500 pc of the Galaxy?}",
      journal = {\mnras},
     keywords = {stars: formation, Galaxy: centre, galaxies: evolution, galaxies: ISM, galaxies: starburst, galaxies: star formation, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = jun,
       volume = {440},
       number = {4},
        pages = {3370-3391},
          doi = {10.1093/mnras/stu494},
archivePrefix = {arXiv},
       eprint = {1303.6286},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.440.3370K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013MNRAS.429..987L,
       author = {{Longmore}, S.~N. and {Bally}, J. and {Testi}, L. and {Purcell}, C.~R. and {Walsh}, A.~J. and {Bressert}, E. and {Pestalozzi}, M. and {Molinari}, S. and {Ott}, J. and {Cortese}, L. and {Battersby}, C. and {Murray}, N. and {Lee}, E. and {Kruijssen}, J.~M.~D. and {Schisano}, E. and {Elia}, D.},
        title = "{Variations in the Galactic star formation rate and density thresholds for star formation}",
      journal = {\mnras},
     keywords = {masers, stars: formation, stars: massive, ISM: clouds, ISM: evolution, Galaxy: centre, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = feb,
       volume = {429},
       number = {2},
        pages = {987-1000},
          doi = {10.1093/mnras/sts376},
archivePrefix = {arXiv},
       eprint = {1208.4256},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.429..987L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2010Natur.463...65C,
       author = {{Crocker}, Roland M. and {Jones}, David I. and {Melia}, Fulvio and {Ott}, J{\"u}rgen and {Protheroe}, Raymond J.},
        title = "{A lower limit of 50 microgauss for the magnetic field near the Galactic Centre}",
      journal = {\nat},
     keywords = {Astrophysics - Galaxy Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2010,
        month = jan,
       volume = {463},
       number = {7277},
        pages = {65-67},
          doi = {10.1038/nature08635},
archivePrefix = {arXiv},
       eprint = {1001.1275},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010Natur.463...65C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017MNRAS.469.2263B,
       author = {{Barnes}, A.~T. and {Longmore}, S.~N. and {Battersby}, C. and {Bally}, J. and {Kruijssen}, J.~M.~D. and {Henshaw}, J.~D. and {Walker}, D.~L.},
        title = "{Star formation rates and efficiencies in the Galactic Centre}",
      journal = {\mnras},
     keywords = {stars: formation, ISM: clouds, H $\lt$sc$\gt$II$\lt$/sc$\gt$ regions, Galaxy: centre, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = aug,
       volume = {469},
       number = {2},
        pages = {2263-2285},
          doi = {10.1093/mnras/stx941},
archivePrefix = {arXiv},
       eprint = {1704.03572},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.469.2263B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...761..156F,
       author = {{Federrath}, Christoph and {Klessen}, Ralf S.},
        title = "{The Star Formation Rate of Turbulent Magnetized Clouds: Comparing Theory, Simulations, and Observations}",
      journal = {\apj},
     keywords = {ISM: clouds, ISM: kinematics and dynamics, ISM: structure, magnetohydrodynamics: MHD, stars: formation, turbulence, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2012,
        month = dec,
       volume = {761},
       number = {2},
          eid = {156},
        pages = {156},
          doi = {10.1088/0004-637X/761/2/156},
archivePrefix = {arXiv},
       eprint = {1209.2856},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...761..156F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014PhR...539...49K,
       author = {{Krumholz}, Mark R.},
        title = "{The big problems in star formation: The star formation rate, stellar clustering, and the initial mass function}",
      journal = {\physrep},
     keywords = {Galaxies: star formation, ISM: clouds, ISM: molecules, Stars: formation, Stars: luminosity function, mass function, Turbulence, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = jun,
       volume = {539},
        pages = {49-134},
          doi = {10.1016/j.physrep.2014.02.001},
archivePrefix = {arXiv},
       eprint = {1402.0867},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014PhR...539...49K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018ApJ...863..118B,
       author = {{Burkhart}, Blakesley},
        title = "{The Star Formation Rate in the Gravoturbulent Interstellar Medium}",
      journal = {\apj},
     keywords = {galaxies: star formation, magnetohydrodynamics: MHD, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = aug,
       volume = {863},
       number = {2},
          eid = {118},
        pages = {118},
          doi = {10.3847/1538-4357/aad002},
archivePrefix = {arXiv},
       eprint = {1801.05428},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...863..118B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hu20,
       author = {{Hu}, Yue and {Lazarian}, A. and {Yuen}, Ka Ho},
        title = "{Velocity Gradient in the Presence of Self-gravity: Identifying Gravity-induced Inflow and Determining Collapsing Stage}",
      journal = {\apj},
     keywords = {845, 1569, 847, 1565, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = jul,
       volume = {897},
       number = {2},
          eid = {123},
        pages = {123},
          doi = {10.3847/1538-4357/ab9948},
archivePrefix = {arXiv},
       eprint = {2002.06754},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...897..123H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1988ApJ...333..729W,
       author = {{Werner}, M.~W. and {Davidson}, J.~A. and {Morris}, M. and {Novak}, G. and {Platt}, S.~R. and {Hildebrand}, R.~H.},
        title = "{The Polarization of the Far-Infrared Radiation from the Galactic Center}",
      journal = {\apj},
     keywords = {Cosmic Dust, Far Infrared Radiation, Galactic Nuclei, Infrared Sources (Astronomy), Linear Polarization, Thermal Emission, H Ii Regions, Interstellar Magnetic Fields, Interstellar Matter, Star Clusters, Astrophysics, GALAXIES: THE GALAXY, GALAXIES: NUCLEI, INFRARED: SOURCES, POLARIZATION},
         year = 1988,
        month = oct,
       volume = {333},
        pages = {729},
          doi = {10.1086/166781},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988ApJ...333..729W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1990IAUS..140..361M,
       author = {{Morris}, Mark},
        title = "{The Magnetic Field in the Inner 70-PARSECS of the Milky-Way}",
     keywords = {Galactic Nuclei, Interstellar Magnetic Fields, Magnetic Field Configurations, Milky Way Galaxy, Molecular Clouds, Radio Frequencies, Ring Currents, Astrophysics},
    booktitle = {Galactic and Intergalactic Magnetic Fields},
         year = 1990,
       editor = {{Beck}, R. and {Kronberg}, P.~P. and {Wielebinski}, R.},
       volume = {140},
        month = jan,
        pages = {361},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1990IAUS..140..361M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...529..241N,
       author = {{Novak}, G. and {Dotson}, J.~L. and {Dowell}, C.~D. and {Hildebrand}, R.~H. and {Renbarger}, T. and {Schleuning}, D.~A.},
        title = "{Submillimeter Polarimetric Observations of the Galactic Center}",
      journal = {\apj},
     keywords = {GALAXY: CENTER, INFRARED: ISM: CONTINUUM, ISM: INDIVIDUAL (SAGITTARIUS A), ISM: MAGNETIC FIELDS, POLARIZATION, Galaxy: Center, Infrared: ISM: Continuum, ISM: individual (Sagittarius A), ISM: Magnetic Fields, Polarization},
         year = 2000,
        month = jan,
       volume = {529},
       number = {1},
        pages = {241-250},
          doi = {10.1086/308231},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...529..241N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005MNRAS.360.1305R,
       author = {{Roy}, Subhashis and {Rao}, A. Pramesh and {Subrahmanyan}, Ravi},
        title = "{Extragalactic sources towards the central region of the Galaxy}",
      journal = {\mnras},
     keywords = {techniques: polarimetric, HII regions, Galaxy: centre, radio continuum: ISM, Astrophysics},
         year = 2005,
        month = jul,
       volume = {360},
       number = {4},
        pages = {1305-1324},
          doi = {10.1111/j.1365-2966.2005.09107.x},
archivePrefix = {arXiv},
       eprint = {0712.0258},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.360.1305R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008A&A...478..435R,
       author = {{Roy}, S. and {Pramesh Rao}, A. and {Subrahmanyan}, R.},
        title = "{Magnetic field near the central region of the Galaxy: rotation measure of extragalactic sources}",
      journal = {\aap},
     keywords = {ISM: magnetic fields, Galaxy: center, techniques: polarimetric, Astrophysics},
         year = 2008,
        month = feb,
       volume = {478},
       number = {2},
        pages = {435-442},
          doi = {10.1051/0004-6361:20066470},
archivePrefix = {arXiv},
       eprint = {0712.0269},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...478..435R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1990ApJ...362..114H,
       author = {{Hildebrand}, R.~H. and {Gonatas}, D.~P. and {Platt}, S.~R. and {Wu}, X.~D. and {Davidson}, J.~A. and {Werner}, M.~W. and {Novak}, G. and {Morris}, M.},
        title = "{The Magnetic Field in the Dust Ring at the Center of the Galaxy}",
      journal = {\apj},
     keywords = {Accretion Disks, Cosmic Dust, Galactic Nuclei, Interstellar Magnetic Fields, Milky Way Galaxy, Ring Structures, Thermal Emission, Angular Momentum, Far Infrared Radiation, Interstellar Matter, Astrophysics, GALAXIES: NUCLEI, GALAXIES: THE GALAXY, INTERSTELLAR: GRAINS, INTERSTELLAR: MAGNETIC FIELDS, POLARIZATION},
         year = 1990,
        month = oct,
       volume = {362},
        pages = {114},
          doi = {10.1086/169248},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1990ApJ...362..114H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2007SPIE.6678E..0DV,
       author = {{Vaillancourt}, John E. and {Chuss}, David T. and {Crutcher}, Richard M. and {Dotson}, Jessie L. and {Dowell}, C. Darren and {Harper}, D. Al and {Hildebrand}, Roger H. and {Jones}, Terry J. and {Lazarian}, Alexandre and {Novak}, Giles and {Werner}, Michael W.},
        title = "{Far-infrared polarimetry from the Stratospheric Observatory for Infrared Astronomy}",
     keywords = {Astrophysics},
    booktitle = {Infrared Spaceborne Remote Sensing and Instrumentation XV},
         year = 2007,
       editor = {{Strojnik-Scholl}, Marija},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {6678},
        month = sep,
          eid = {66780D},
        pages = {66780D},
          doi = {10.1117/12.730922},
archivePrefix = {arXiv},
       eprint = {0711.3047},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007SPIE.6678E..0DV},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2020arXiv200207996L,
       author = {{Lazarian}, Alex and {Yuen}, Ka Ho and {Pogosyan}, Dmitri},
        title = "{Obtaining magnetic field strength using differential measure approach and velocity channel maps}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = feb,
          eid = {arXiv:2002.07996},
        pages = {arXiv:2002.07996},
archivePrefix = {arXiv},
       eprint = {2002.07996},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv200207996L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kspace,
       author = {{Hu}, Yue, and {Lazarian}, Alex},
        title = "{Tracing Magnetic Fields with the Gradient Technique: Spatial Filtering and Use of Interferometers}",
      journal = {submitted to ApJ},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2022,
        month = Mar.,
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019arXiv190403173Y,
       author = {{Yuen}, Ka Ho and {Hu}, Yue and {Lazarian}, A. and {Pogosyan}, D.},
        title = "{Comment on Clark et al. (2019) ``The Physical Nature of Neutral Hydrogen Intensity Structure''}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = apr,
          eid = {arXiv:1904.03173},
        pages = {arXiv:1904.03173},
archivePrefix = {arXiv},
       eprint = {1904.03173},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190403173Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1979cmft.book.....P,
       author = {{Parker}, E.~N.},
        title = "{Cosmical magnetic fields. Their origin and their activity}",
         year = 1979,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1979cmft.book.....P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{LY18a,
       author = {{Lazarian}, A. and {Yuen}, Ka Ho},
        title = "{Tracing Magnetic Fields with Spectroscopic Channel Maps}",
      journal = {\apj},
     keywords = {ISM: magnetic fields, ISM: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = jan,
       volume = {853},
       number = {1},
          eid = {96},
        pages = {96},
          doi = {10.3847/1538-4357/aaa241},
archivePrefix = {arXiv},
       eprint = {1703.03119},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...853...96L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ARA&A..53..501A,
       author = {{Andersson}, B. -G. and {Lazarian}, A. and {Vaillancourt}, John E.},
        title = "{Interstellar Dust Grain Alignment}",
      journal = {\araa},
         year = 2015,
        month = aug,
       volume = {53},
        pages = {501-539},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ARA&A..53..501A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2007ApJ...669L..77L,
       author = {{Lazarian}, A. and {Hoang}, Thiem},
        title = "{Subsonic Mechanical Alignment of Irregular Grains}",
      journal = {\apjl},
     keywords = {ISM: Dust, Extinction, ISM: Magnetic Fields, Polarization, Astrophysics},
         year = 2007,
        month = nov,
       volume = {669},
       number = {2},
        pages = {L77-L80},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...669L..77L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018JAI.....740008H,
       author = {{Harper}, Doyal A. and {Runyan}, Marcus C. and {Dowell}, C. Darren and {Wirth}, C. Jesse and {Amato}, Michael and {Ames}, Troy and {Amiri}, Mandana and {Banks}, Stuart and {Bartels}, Arlin and {Benford}, Dominic J. and {Berthoud}, Marc and {Buchanan}, Ernest and {Casey}, Sean and {Chapman}, Nicholas L. and {Chuss}, David T. and {Cook}, Brant and {Derro}, Rebecca and {Dotson}, Jessie L. and {Evans}, Rhodri and {Fixsen}, Dale and {Gatley}, Ian and {Guerra}, Jordan A. and {Halpern}, Mark and {Hamilton}, Ryan T. and {Hamlin}, Louise A. and {Hansen}, Christopher J. and {Heimsath}, Stephen and {Hermida}, Alfonso and {Hilton}, Gene C. and {Hirsch}, Robert and {Hollister}, Matthew I. and {Hostetter}, Carl F. and {Irwin}, Kent and {Jhabvala}, Christine A. and {Jhabvala}, Murzban and {Kastner}, Joel and {Kov{\'a}cs}, Attila and {Lin}, Sean and {Loewenstein}, Robert F. and {Looney}, Leslie W. and {Lopez-Rodriguez}, Enrique and {Maher}, Stephen F. and {Michail}, Joseph M. and {Miller}, Timothy M. and {Moseley}, S. Harvey and {Novak}, Giles and {Pernic}, Robert J. and {Rennick}, Timothy and {Rhody}, Harvey and {Sandberg}, Eric and {Sandford}, Dale and {Santos}, Fabio Pereira and {Shafer}, Rick and {Sharp}, Elmer H. and {Shirron}, Peter and {Siah}, Javad and {Silverberg}, Robert and {Sparr}, Leroy M. and {Spotz}, Robert and {Staguhn}, Johannes G. and {Toorian}, Armen S. and {Towey}, Shannon and {Tuttle}, Jim and {Vaillancourt}, John and {Voellmer}, George and {Volpert}, Carolyn G. and {Wang}, Shu-I. and {Wollack}, Edward J.},
        title = "{HAWC+, the Far-Infrared Camera and Polarimeter for SOFIA}",
      journal = {Journal of Astronomical Instrumentation},
     keywords = {Instrumentation, polarimeters, camera, far-infrared, detectors, stars, formation, dust},
         year = 2018,
        month = jan,
       volume = {7},
       number = {4},
          eid = {1840008-1025},
        pages = {1840008-1025},
          doi = {10.1142/S2251171718400081},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018JAI.....740008H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015A&A...576A.104P,
       author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and {Alina}, D. and {Alves}, M.~I.~R. and {Armitage-Caplan}, C. and {Arnaud}, M. and {Arzoumanian}, D. and {Ashdown}, M. and {Atrio-Barandela}, F. and {Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Battaner}, E. and {Benabed}, K. and {Benoit-L{\'e}vy}, A. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bracco}, A. and {Burigana}, C. and {Butler}, R.~C. and {Cardoso}, J. -F. and {Catalano}, A. and {Chamballu}, A. and {Chary}, R. -R. and {Chiang}, H.~C. and {Christensen}, P.~R. and {Colombi}, S. and {Colombo}, L.~P.~L. and {Combet}, C. and {Couchot}, F. and {Coulais}, A. and {Crill}, B.~P. and {Curto}, A. and {Cuttaia}, F. and {Danese}, L. and {Davies}, R.~D. and {Davis}, R.~J. and {de Bernardis}, P. and {de Gouveia Dal Pino}, E.~M. and {de Rosa}, A. and {de Zotti}, G. and {Delabrouille}, J. and {D{\'e}sert}, F. -X. and {Dickinson}, C. and {Diego}, J.~M. and {Donzelli}, S. and {Dor{\'e}}, O. and {Douspis}, M. and {Dunkley}, J. and {Dupac}, X. and {Efstathiou}, G. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Falgarone}, E. and {Ferri{\`e}re}, K. and {Finelli}, F. and {Forni}, O. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Galeotta}, S. and {Ganga}, K. and {Ghosh}, T. and {Giard}, M. and {Giraud-H{\'e}raud}, Y. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gregorio}, A. and {Gruppuso}, A. and {Guillet}, V. and {Hansen}, F.~K. and {Harrison}, D.~L. and {Helou}, G. and {Hern{\'a}ndez-Monteagudo}, C. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Hobson}, M. and {Holmes}, W.~A. and {Hornstrup}, A. and {Huffenberger}, K.~M. and {Jaffe}, A.~H. and {Jaffe}, T.~R. and {Jones}, W.~C. and {Juvela}, M. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kisner}, T.~S. and {Kneissl}, R. and {Knoche}, J. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {L{\"a}hteenm{\"a}ki}, A. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lawrence}, C.~R. and {Leahy}, J.~P. and {Leonardi}, R. and {Levrier}, F. and {Liguori}, M. and {Lilje}, P.~B. and {Linden-V{\o}rnle}, M. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maffei}, B. and {Magalh{\~a}es}, A.~M. and {Maino}, D. and {Mandolesi}, N. and {Maris}, M. and {Marshall}, D.~J. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Matarrese}, S. and {Mazzotta}, P. and {Melchiorri}, A. and {Mendes}, L. and {Mennella}, A. and {Migliaccio}, M. and {Miville-Desch{\^e}nes}, M. -A. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Mortlock}, D. and {Munshi}, D. and {Murphy}, J.~A. and {Naselsky}, P. and {Nati}, F. and {Natoli}, P. and {Netterfield}, C.~B. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {Oxborrow}, C.~A. and {Pagano}, L. and {Pajot}, F. and {Paladini}, R. and {Paoletti}, D. and {Pasian}, F. and {Pearson}, T.~J. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Piacentini}, F. and {Piat}, M. and {Pietrobon}, D. and {Plaszczynski}, S. and {Poidevin}, F. and {Pointecouteau}, E. and {Polenta}, G. and {Popa}, L. and {Pratt}, G.~W. and {Prunet}, S. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reach}, W.~T. and {Rebolo}, R. and {Reinecke}, M. and {Remazeilles}, M. and {Renault}, C. and {Ricciardi}, S. and {Riller}, T. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Rusholme}, B. and {Sandri}, M. and {Savini}, G. and {Scott}, D. and {Spencer}, L.~D. and {Stolyarov}, V. and {Stompor}, R. and {Sudiwala}, R. and {Sutton}, D. and {Suur-Uski}, A. -S. and {Sygnet}, J. -F. and {Tauber}, J.~A. and {Terenzi}, L. and {Toffolatti}, L. and {Tomasi}, M. and {Tristram}, M. and {Tucci}, M. and {Umana}, G. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, B. and {Vielva}, P. and {Villa}, F. and {Wade}, L.~A. and {Wandelt}, B.~D. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck intermediate results. XIX. An overview of the polarized thermal emission from Galactic dust}",
      journal = {\aap},
     keywords = {ISM: general, dust, extinction, ISM: magnetic fields, ISM:, clouds, submillimeter: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = apr,
       volume = {576},
          eid = {A104},
        pages = {A104},
          doi = {10.1051/0004-6361/201424082},
archivePrefix = {arXiv},
       eprint = {1405.0871},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...576A.104P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1986AJ.....92..818T,
       author = {{Tsuboi}, M. and {Inoue}, M. and {Handa}, T. and {Tabara}, H. and {Kato}, T. and {Sofue}, Y. and {Kaifu}, N.},
        title = "{Prominent polarized plumes in the Galactic Center region and their magnetic field.}",
      journal = {\aj},
     keywords = {Galactic Nuclei, Interstellar Magnetic Fields, Linear Polarization, Milky Way Galaxy, Radio Astronomy, Depolarization, Magnetic Field Configurations, Plumes, Polarization Characteristics, Astrophysics},
         year = 1986,
        month = oct,
       volume = {92},
        pages = {818-824},
          doi = {10.1086/114215},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1986AJ.....92..818T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1990IAUS..140..361M,
       author = {{Morris}, Mark},
        title = "{The Magnetic Field in the Inner 70-PARSECS of the Milky-Way}",
     keywords = {Galactic Nuclei, Interstellar Magnetic Fields, Magnetic Field Configurations, Milky Way Galaxy, Molecular Clouds, Radio Frequencies, Ring Currents, Astrophysics},
    booktitle = {Galactic and Intergalactic Magnetic Fields},
         year = 1990,
       editor = {{Beck}, R. and {Kronberg}, P.~P. and {Wielebinski}, R.},
       volume = {140},
        month = jan,
        pages = {361},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1990IAUS..140..361M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999ApJ...521L..41L,
       author = {{Lang}, Cornelia C. and {Anantharamaiah}, K.~R. and {Kassim}, N.~E. and {Lazio}, T.~J.~W.},
        title = "{Discovery of a Nonthermal Galactic Center Filament (G358.85+0.47) Parallel to the Galactic Plane}",
      journal = {\apjl},
     keywords = {GALAXY: CENTER, ISM: MAGNETIC FIELDS, RADIO CONTINUUM: ISM, Galaxy: Center, ISM: Magnetic Fields, Radio Continuum: ISM, Astrophysics},
         year = 1999,
        month = aug,
       volume = {521},
       number = {1},
        pages = {L41-L44},
          doi = {10.1086/312180},
archivePrefix = {arXiv},
       eprint = {astro-ph/9906285},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...521L..41L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019ApJ...884..170P,
       author = {{Par{\'e}}, Dylan M. and {Lang}, Cornelia C. and {Morris}, Mark R. and {Moore}, Hailey and {Mao}, Sui Ann},
        title = "{A VLA Polarimetric Study of the Galactic Center Radio Arc: Characterizing Polarization, Rotation Measure, and Magnetic Field Properties}",
      journal = {\apj},
     keywords = {Galactic center, Galaxy magnetic fields, Milky Way magnetic fields, Interstellar synchrotron emission, Radio astronomy, Very Large Array, Radio continuum emission, Non-thermal radiation sources, 565, 604, 1057, 856, 1338, 1766, 1340, 1119, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = oct,
       volume = {884},
       number = {2},
          eid = {170},
        pages = {170},
          doi = {10.3847/1538-4357/ab45ed},
archivePrefix = {arXiv},
       eprint = {1909.08268},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...884..170P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PCA,
       author = {{Hu}, Yue and {Yuen}, Ka Ho and {Lazarian}, A.},
        title = "{Improving the accuracy of magnetic field tracing by velocity gradients: principal component analysis}",
      journal = {\mnras},
     keywords = {magnetohydrodynamics (MHD), turbulence, methods: numerical, ISM: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = oct,
       volume = {480},
       number = {1},
        pages = {1333-1339},
          doi = {10.1093/mnras/sty1807},
archivePrefix = {arXiv},
       eprint = {1802.08772},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.480.1333H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GS95,
       author = {{Goldreich}, P. and {Sridhar}, S.},
        title = "{Toward a Theory of Interstellar Turbulence. II. Strong Alfvenic Turbulence}",
      journal = {\apj},
     keywords = {Interstellar Space, Magnetic Fields, Magnetohydrodynamic Turbulence, Magnetohydrodynamic Waves, Electron Density (Concentration), Energy Spectra, Radio Waves, Variations, Wave Scattering, Astrophysics, ISM: GENERAL, MAGNETOHYDRODYNAMICS: MHD, TURBULENCE},
         year = 1995,
        month = jan,
       volume = {438},
        pages = {763},
          doi = {10.1086/175121},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...438..763G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LV99,
       author = {{Lazarian}, A. and {Vishniac}, Ethan T.},
        title = "{Reconnection in a Weakly Stochastic Field}",
      journal = {\apj},
     keywords = {GALAXIES: MAGNETIC FIELDS, MAGNETOHYDRODYNAMICS: MHD, Galaxies: Magnetic Fields, Magnetohydrodynamics: MHD, Astrophysics, Physics - Fluid Dynamics, Physics - Geophysics, Physics - Plasma Physics, Physics - Space Physics},
         year = 1999,
        month = jun,
       volume = {517},
       number = {2},
        pages = {700-718},
          doi = {10.1086/307233},
archivePrefix = {arXiv},
       eprint = {astro-ph/9811037},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...517..700L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2021ApJ...911...37H,
       author = {{Hu}, Yue and {Xu}, Siyao and {Lazarian}, A.},
        title = "{Anisotropies in Compressible MHD Turbulence: Probing Magnetic Fields and Measuring Magnetization}",
      journal = {\apj},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, 847, 845, 839, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = apr,
       volume = {911},
       number = {1},
          eid = {37},
        pages = {37},
          doi = {10.3847/1538-4357/abea18},
archivePrefix = {arXiv},
       eprint = {2012.06039},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...911...37H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018arXiv180200024Y,
       author = {{Yuen}, Ka Ho and {Lazarian}, A.},
        title = "{Advancing the Velocity Gradient Technique: Using Gradient Amplitudes and handling thermal broadening}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jan,
          eid = {arXiv:1802.00024},
        pages = {arXiv:1802.00024},
archivePrefix = {arXiv},
       eprint = {1802.00024},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv180200024Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...740..117E,
       author = {{Esquivel}, A. and {Lazarian}, A.},
        title = "{Velocity Anisotropy as a Diagnostic of the Magnetization of the Interstellar Medium and Molecular Clouds}",
      journal = {\apj},
     keywords = {ISM: general, ISM: structure, magnetohydrodynamics: MHD, radio lines: ISM, turbulence, Astrophysics - Astrophysics of Galaxies},
         year = 2011,
        month = oct,
       volume = {740},
       number = {2},
          eid = {117},
        pages = {117},
          doi = {10.1088/0004-637X/740/2/117},
archivePrefix = {arXiv},
       eprint = {1108.0693},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...740..117E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021ApJ...910...88X,
       author = {{Xu}, Siyao and {Hu}, Yue},
        title = "{Measuring Magnetization with Rotation Measures and Velocity Centroids in Supersonic MHD Turbulence}",
      journal = {\apj},
     keywords = {Interstellar medium, Magnetohydrodynamics, Interstellar magnetic fields, 847, 1964, 845, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = apr,
       volume = {910},
       number = {2},
          eid = {88},
        pages = {88},
          doi = {10.3847/1538-4357/abe403},
archivePrefix = {arXiv},
       eprint = {2102.05647},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...910...88X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021ApJ...915...67H,
       author = {{Hu}, Yue and {Lazarian}, A. and {Xu}, Siyao},
        title = "{Anisotropic Turbulence in Position-Position-Velocity Space: Probing Three-dimensional Magnetic Fields}",
      journal = {\apj},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, 847, 845, 839, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = jul,
       volume = {915},
       number = {1},
          eid = {67},
        pages = {67},
          doi = {10.3847/1538-4357/ac00ab},
archivePrefix = {arXiv},
       eprint = {2104.02842},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...915...67H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018ApJ...865...46L,
       author = {{Lazarian}, A. and {Yuen}, Ka Ho and {Ho}, Ka Wai and {Chen}, Junda and {Lazarian}, Victor and {Lu}, Zekun and {Yang}, Bo and {Hu}, Yue},
        title = "{Distribution of Velocity Gradient Orientations: Mapping Magnetization with the Velocity Gradient Technique}",
      journal = {\apj},
     keywords = {ISM: general, ISM: structure, magnetohydrodynamics: MHD, radio continuum: ISM, turbulence, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = sep,
       volume = {865},
       number = {1},
          eid = {46},
        pages = {46},
          doi = {10.3847/1538-4357/aad7ff},
archivePrefix = {arXiv},
       eprint = {1802.02984},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...865...46L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021ApJ...911...37H,
       author = {{Hu}, Yue and {Xu}, Siyao and {Lazarian}, A.},
        title = "{Anisotropies in Compressible MHD Turbulence: Probing Magnetic Fields and Measuring Magnetization}",
      journal = {\apj},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, 847, 845, 839, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = apr,
       volume = {911},
       number = {1},
          eid = {37},
        pages = {37},
          doi = {10.3847/1538-4357/abea18},
archivePrefix = {arXiv},
       eprint = {2012.06039},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...911...37H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021ApJ...915...67H,
       author = {{Hu}, Yue and {Lazarian}, A. and {Xu}, Siyao},
        title = "{Anisotropic Turbulence in Position-Position-Velocity Space: Probing Three-dimensional Magnetic Fields}",
      journal = {\apj},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, 847, 845, 839, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = jul,
       volume = {915},
       number = {1},
          eid = {67},
        pages = {67},
          doi = {10.3847/1538-4357/ac00ab},
archivePrefix = {arXiv},
       eprint = {2104.02842},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...915...67H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015MNRAS.451..372R,
       author = {{Robitaille}, J. -F. and {Scaife}, A.~M.~M.},
        title = "{Multiscale analysis of the gradient of linear polarization}",
      journal = {\mnras},
     keywords = {methods: statistical, techniques: image processing, ISM: general, ISM: magnetic fields, ISM: structure, radio continuum: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = jul,
       volume = {451},
       number = {1},
        pages = {372-382},
          doi = {10.1093/mnras/stv920},
archivePrefix = {arXiv},
       eprint = {1504.06217},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.451..372R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017MNRAS.468.2957R,
       author = {{Robitaille}, J. -F. and {Scaife}, A.~M.~M. and {Carretti}, E. and {Gaensler}, B.~M. and {McEwen}, J.~D. and {Leistedt}, B. and {Haverkorn}, M. and {Bernardi}, G. and {Kesteven}, M.~J. and {Poppi}, S. and {Staveley-Smith}, L.},
        title = "{A new perspective on turbulent Galactic magnetic fields through comparison of linear polarization decomposition techniques}",
      journal = {\mnras},
     keywords = {techniques: image processing, ISM: general, ISM: magnetic fields, ISM: structure, radio continuum: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = jul,
       volume = {468},
       number = {3},
        pages = {2957-2974},
          doi = {10.1093/mnras/stx642},
archivePrefix = {arXiv},
       eprint = {1703.04469},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.468.2957R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...749..145B,
       author = {{Burkhart}, Blakesley and {Lazarian}, A. and {Gaensler}, B.~M.},
        title = "{Properties of Interstellar Turbulence from Gradients of Linear Polarization Maps}",
      journal = {\apj},
     keywords = {ISM: general, magnetohydrodynamics: MHD, polarization, shock waves, turbulence, Astrophysics - Astrophysics of Galaxies},
         year = 2012,
        month = apr,
       volume = {749},
       number = {2},
          eid = {145},
        pages = {145},
          doi = {10.1088/0004-637X/749/2/145},
archivePrefix = {arXiv},
       eprint = {1111.3544},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...749..145B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2020NatAs...4.1064H,
       author = {{Henshaw}, Jonathan D. and {Kruijssen}, J.~M. Diederik and {Longmore}, Steven N. and {Riener}, Manuel and {Leroy}, Adam K. and {Rosolowsky}, Erik and {Ginsburg}, Adam and {Battersby}, Cara and {Chevance}, M{\'e}lanie and {Meidt}, Sharon E. and {Glover}, Simon C.~O. and {Hughes}, Annie and {Kainulainen}, Jouni and {Klessen}, Ralf S. and {Schinnerer}, Eva and {Schruba}, Andreas and {Beuther}, Henrik and {Bigiel}, Frank and {Blanc}, Guillermo A. and {Emsellem}, Eric and {Henning}, Thomas and {Herrera}, Cynthia N. and {Koch}, Eric W. and {Pety}, J{\'e}r{\^o}me and {Ragan}, Sarah E. and {Sun}, Jiayi},
        title = "{Ubiquitous velocity fluctuations throughout the molecular interstellar medium}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jul,
       volume = {4},
        pages = {1064-1071},
          doi = {10.1038/s41550-020-1126-z},
archivePrefix = {arXiv},
       eprint = {2007.01877},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020NatAs...4.1064H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2011Natur.478..214G,
       author = {{Gaensler}, B.~M. and {Haverkorn}, M. and {Burkhart}, B. and {Newton-McGee}, K.~J. and {Ekers}, R.~D. and {Lazarian}, A. and {McClure-Griffiths}, N.~M. and {Robishaw}, T. and {Dickey}, J.~M. and {Green}, A.~J.},
        title = "{Low-Mach-number turbulence in interstellar gas revealed by radio polarization gradients}",
      journal = {\nat},
     keywords = {Astrophysics - Galaxy Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics, Physics - Computational Physics, Physics - Fluid Dynamics},
         year = 2011,
        month = oct,
       volume = {478},
       number = {7368},
        pages = {214-217},
          doi = {10.1038/nature10446},
archivePrefix = {arXiv},
       eprint = {1110.2896},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011Natur.478..214G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Liu21,
       author = {{Liu}, Mingrui and {Hu}, Yue and {Lazarian}, Alex},
        title = "{Velocity Gradients: Magnetic Field Tomography towards the Supernova Remnant W44}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = sep,
          eid = {arXiv:2109.13670},
        pages = {arXiv:2109.13670},
archivePrefix = {arXiv},
       eprint = {2109.13670},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210913670L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019A&A...630A..74M,
       author = {{Mangilli}, A. and {Aumont}, J. and {Bernard}, J. -Ph. and {Buzzelli}, A. and {de Gasperis}, G. and {Durrive}, J.~B. and {Ferriere}, K. and {Fo{\"e}nard}, G. and {Hughes}, A. and {Lacourt}, A. and {Misawa}, R. and {Montier}, L. and {Mot}, B. and {Ristorcelli}, I. and {Roussel}, H. and {Ade}, P. and {Alina}, D. and {de Bernardis}, P. and {de Gouveia Dal Pino}, E. and {Dubois}, J.~P. and {Engel}, C. and {Guillet}, V. and {Hargrave}, P. and {Laureijs}, R. and {Longval}, Y. and {Maffei}, B. and {Magalhaes}, A.~M. and {Marty}, C. and {Masi}, S. and {Montel}, J. and {Pajot}, F. and {P{\'e}rot}, E. and {Rodriguez}, L. and {Salatino}, M. and {Saccoccio}, M. and {Savini}, G. and {Stever}, S. and {Tauber}, J. and {Tibbs}, C. and {Tucker}, C.},
        title = "{The geometry of the magnetic field in the central molecular zone measured by PILOT}",
      journal = {\aap},
     keywords = {Galaxy: center, polarization, magnetic fields, balloons, methods: data analysis, dust, extinction, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = oct,
       volume = {630},
          eid = {A74},
        pages = {A74},
          doi = {10.1051/0004-6361/201935072},
archivePrefix = {arXiv},
       eprint = {1901.06196},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...630A..74M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2009A&A...505.1183F,
       author = {{Ferri{\`e}re}, K.},
        title = "{Interstellar magnetic fields in the Galactic center region}",
      journal = {\aap},
     keywords = {ISM: magnetic fields, ISM: general, ISM: structure, cosmic rays, Galaxy: center, galaxies: magnetic fields, Astrophysics - Astrophysics of Galaxies},
         year = 2009,
        month = oct,
       volume = {505},
       number = {3},
        pages = {1183-1198},
          doi = {10.1051/0004-6361/200912617},
archivePrefix = {arXiv},
       eprint = {0908.2037},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&A...505.1183F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1999ASPC..186..519S,
       author = {{Sofue}, Y. and {Lang}, C.~C.},
        title = "{The Magnetic Field in the Galactic Center}",
    booktitle = {The Central Parsecs of the Galaxy},
         year = 1999,
       editor = {{Falcke}, Heino and {Cotera}, Angela and {Duschl}, Wolfgang J. and {Melia}, Fulvio and {Rieke}, Marcia J.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {186},
        month = jun,
        pages = {519},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ASPC..186..519S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



==> reference <==
@ARTICLE{2015A&A...576A.105P,
       author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and {Alina}, D. and {Alves}, M.~I.~R. and {Aniano}, G. and {Armitage-Caplan}, C. and {Arnaud}, M. and {Arzoumanian}, D. and {Ashdown}, M. and {Atrio-Barandela}, F. and {Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Battaner}, E. and {Benabed}, K. and {Benoit-L{\'e}vy}, A. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bracco}, A. and {Burigana}, C. and {Cardoso}, J. -F. and {Catalano}, A. and {Chamballu}, A. and {Chiang}, H.~C. and {Christensen}, P.~R. and {Colombi}, S. and {Colombo}, L.~P.~L. and {Combet}, C. and {Couchot}, F. and {Coulais}, A. and {Crill}, B.~P. and {Curto}, A. and {Cuttaia}, F. and {Danese}, L. and {Davies}, R.~D. and {Davis}, R.~J. and {de Bernardis}, P. and {de Rosa}, A. and {de Zotti}, G. and {Delabrouille}, J. and {Dickinson}, C. and {Diego}, J.~M. and {Donzelli}, S. and {Dor{\'e}}, O. and {Douspis}, M. and {Dupac}, X. and {Efstathiou}, G. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Falgarone}, E. and {Fanciullo}, L. and {Ferri{\`e}re}, K. and {Finelli}, F. and {Forni}, O. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Galeotta}, S. and {Ganga}, K. and {Ghosh}, T. and {Giard}, M. and {Giraud-H{\'e}raud}, Y. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gregorio}, A. and {Gruppuso}, A. and {Guillet}, V. and {Hansen}, F.~K. and {Harrison}, D.~L. and {Helou}, G. and {Hern{\'a}ndez-Monteagudo}, C. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Hobson}, M. and {Holmes}, W.~A. and {Hornstrup}, A. and {Huffenberger}, K.~M. and {Jaffe}, A.~H. and {Jaffe}, T.~R. and {Jones}, W.~C. and {Juvela}, M. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kisner}, T.~S. and {Kneissl}, R. and {Knoche}, J. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lawrence}, C.~R. and {Leonardi}, R. and {Levrier}, F. and {Liguori}, M. and {Lilje}, P.~B. and {Linden-V{\o}rnle}, M. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maino}, D. and {Mandolesi}, N. and {Maris}, M. and {Marshall}, D.~J. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Matarrese}, S. and {Mazzotta}, P. and {Melchiorri}, A. and {Mendes}, L. and {Mennella}, A. and {Migliaccio}, M. and {Miville-Desch{\^e}nes}, M. -A. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Mortlock}, D. and {Munshi}, D. and {Murphy}, J.~A. and {Naselsky}, P. and {Nati}, F. and {Natoli}, P. and {Netterfield}, C.~B. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {Oxborrow}, C.~A. and {Pagano}, L. and {Pajot}, F. and {Paoletti}, D. and {Pasian}, F. and {Pelkonen}, V. -M. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Piacentini}, F. and {Piat}, M. and {Pietrobon}, D. and {Plaszczynski}, S. and {Pointecouteau}, E. and {Polenta}, G. and {Popa}, L. and {Pratt}, G.~W. and {Prunet}, S. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reinecke}, M. and {Remazeilles}, M. and {Renault}, C. and {Ricciardi}, S. and {Riller}, T. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rusholme}, B. and {Sandri}, M. and {Scott}, D. and {Soler}, J.~D. and {Spencer}, L.~D. and {Stolyarov}, V. and {Stompor}, R. and {Sudiwala}, R. and {Sutton}, D. and {Suur-Uski}, A. -S. and {Sygnet}, J. -F. and {Tauber}, J.~A. and {Terenzi}, L. and {Toffolatti}, L. and {Tomasi}, M. and {Tristram}, M. and {Tucci}, M. and {Umana}, G. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, B. and {Vielva}, P. and {Villa}, F. and {Wade}, L.~A. and {Wandelt}, B.~D. and {Zonca}, A.},
        title = "{Planck intermediate results. XX. Comparison of polarized thermal emission from Galactic dust with simulations of MHD turbulence}",
      journal = {\aap},
     keywords = {ISM: general, dust, extinction, ISM: magnetic fields, ISM:, clouds, infrared: ISM, submillimeter: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = apr,
       volume = {576},
          eid = {A105},
        pages = {A105},
          doi = {10.1051/0004-6361/201424086},
archivePrefix = {arXiv},
       eprint = {1405.0872},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...576A.105P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2016MNRAS.457.2675H,
       author = {{Henshaw}, J.~D. and {Longmore}, S.~N. and {Kruijssen}, J.~M.~D. and {Davies}, B. and {Bally}, J. and {Barnes}, A. and {Battersby}, C. and {Burton}, M. and {Cunningham}, M.~R. and {Dale}, J.~E. and {Ginsburg}, A. and {Immer}, K. and {Jones}, P.~A. and {Kendrew}, S. and {Mills}, E.~A.~C. and {Molinari}, S. and {Moore}, T.~J.~T. and {Ott}, J. and {Pillai}, T. and {Rathborne}, J. and {Schilke}, P. and {Schmiedeke}, A. and {Testi}, L. and {Walker}, D. and {Walsh}, A. and {Zhang}, Q.},
        title = "{Molecular gas kinematics within the central 250 pc of the Milky Way}",
      journal = {\mnras},
     keywords = {stars: formation, ISM: clouds, ISM: kinematics and dynamics, ISM: structure, Galaxy: centre, galaxies: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = apr,
       volume = {457},
       number = {3},
        pages = {2675-2702},
          doi = {10.1093/mnras/stw121},
archivePrefix = {arXiv},
       eprint = {1601.03732},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.457.2675H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999ARA&A..37...37K,
       author = {{Kulsrud}, Russell M.},
        title = "{A Critical Review of Galactic Dynamos}",
      journal = {\araa},
     keywords = {MHD DYNAMOS, GALACTIC MAGNETIC FIELDS, ALPHA EFFECT, FLUX EXPULSION, SMALL-SCALE FIELDS},
         year = 1999,
        month = jan,
       volume = {37},
        pages = {37-64},
          doi = {10.1146/annurev.astro.37.1.37},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ARA&A..37...37K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002ApJ...564..291C,
       author = {{Cho}, Jungyeon and {Lazarian}, Alex and {Vishniac}, Ethan T.},
        title = "{Simulations of Magnetohydrodynamic Turbulence in a Strongly Magnetized Medium}",
      journal = {\apj},
     keywords = {ISM: General, Methods: Numerical, Magnetohydrodynamics: MHD, Turbulence, Astrophysics},
         year = 2002,
        month = jan,
       volume = {564},
       number = {1},
        pages = {291-301},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...564..291C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992A&A...264..326L,
       author = {{Lazarian}, Alexander},
        title = "{Diffusion-generated electromotive force and seed magnetic field problem}",
      journal = {\aap},
     keywords = {Electromotive Forces, Galactic Evolution, Interstellar Magnetic Fields, Magnetic Diffusion, Computational Astrophysics, Cosmic Plasma, Interstellar Gas, Ionized Gases, Astrophysics},
         year = 1992,
        month = oct,
       volume = {264},
       number = {1},
        pages = {326-330},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992A&A...264..326L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1988ASSL..133.....R,
       author = {{Ruzmaikin}, Aleksandr A. and {Sokolov}, Dmitrii D. and {Shukurov}, Anvar M.},
        title = "{Magnetic Fields of Galaxies}",
         year = 1988,
       volume = {133},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988ASSL..133.....R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994PhRvL..72.1651G,
       author = {{Gruzinov}, A.~V. and {Diamond}, P.~H.},
        title = "{Self-consistent theory of mean-field electrodynamics}",
      journal = {\prl},
     keywords = {47.65.+a, 03.50.De, 91.25.Cw, Classical electromagnetism Maxwell equations, Origins and models of the magnetic field, dynamo theories},
         year = 1994,
        month = mar,
       volume = {72},
       number = {11},
        pages = {1651-1653},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994PhRvL..72.1651G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...550..752V,
       author = {{Vishniac}, Ethan T. and {Cho}, Jungyeon},
        title = "{Magnetic Helicity Conservation and Astrophysical Dynamos}",
      journal = {\apj},
     keywords = {ISM: Magnetic Fields, Magnetic Fields, Magnetohydrodynamics: MHD, Turbulence, Astrophysics, Physics - Plasma Physics},
         year = 2001,
        month = apr,
       volume = {550},
       number = {2},
        pages = {752-760},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...550..752V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...780..144V,
       author = {{Vishniac}, Ethan T. and {Shapovalov}, Dmitry},
        title = "{Properties of Magnetic Helicity Flux in Turbulent Dynamos}",
      journal = {\apj},
     keywords = {ISM: general, magnetic fields, magnetohydrodynamics: MHD, turbulence},
         year = 2014,
        month = jan,
       volume = {780},
       number = {2},
          eid = {144},
        pages = {144},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...780..144V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021MNRAS.503.1290S,
       author = {{Santos-Lima}, R. and {Guerrero}, G. and {de Gouveia Dal Pino}, E.~M. and {Lazarian}, A.},
        title = "{Diffusion of large-scale magnetic fields by reconnection in MHD turbulence}",
      journal = {\mnras},
     keywords = {magnetic fields, magnetic reconnection, MHD, turbulence, methods: numerical, stars: formation, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = may,
       volume = {503},
       number = {1},
        pages = {1290-1309},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.503.1290S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@INPROCEEDINGS{2015ASSL..407..311L,
       author = {{Lazarian}, Alex and {Eyink}, Gregory L. and {Vishniac}, Ethan T. and {Kowal}, Grzegorz},
        title = "{Magnetic Reconnection in Astrophysical Environments}",
     keywords = {Physics, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Physics - Plasma Physics, Physics - Space Physics},
    booktitle = {Magnetic Fields in Diffuse Media},
         year = 2015,
       editor = {{Lazarian}, Alexander and {de Gouveia Dal Pino}, Elisabete M. and {Melioli}, Claudio},
       series = {Astrophysics and Space Science Library},
       volume = {407},
        month = jan,
        pages = {311},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ASSL..407..311L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1971ApJ...163..255P,
       author = {{Parker}, E.~N.},
        title = "{The Generation of Magnetic Fields in Astrophysical Bodies. II. The Galactic Field}",
      journal = {\apj},
         year = 1971,
        month = jan,
       volume = {163},
        pages = {255},
          doi = {10.1086/150765},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1971ApJ...163..255P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...528..723C,
       author = {{Chandran}, Benjamin D.~G. and {Cowley}, Steve C. and {Morris}, Mark},
        title = "{Magnetic Flux Accumulation at the Galactic Center and Its Implications for the Strength of the Pregalactic Magnetic Field}",
      journal = {\apj},
     keywords = {DIFFUSION, GALAXY: CENTER, GALAXY: EVOLUTION, MAGNETOHYDRODYNAMICS: MHD, ISM: MAGNETIC FIELDS, TURBULENCE, Diffusion, Galaxy: Center, Galaxy: Evolution, Magnetohydrodynamics: MHD, ISM: Magnetic Fields, Turbulence},
         year = 2000,
        month = jan,
       volume = {528},
       number = {2},
        pages = {723-733},
          doi = {10.1086/308184},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...528..723C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1974PASJ...26..117K,
       author = {{Kaifu}, N. and {Iguchi}, T. and {Kato}, T.},
        title = "{Gaseous Structure in the Galactic Center Region}",
      journal = {PASJ},
         year = 1974,
        month = jan,
       volume = {26},
        pages = {117},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1974PASJ...26..117K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2016MNRAS.457.2675H,
       author = {{Henshaw}, J.~D. and {Longmore}, S.~N. and {Kruijssen}, J.~M.~D. and {Davies}, B. and {Bally}, J. and {Barnes}, A. and {Battersby}, C. and {Burton}, M. and {Cunningham}, M.~R. and {Dale}, J.~E. and {Ginsburg}, A. and {Immer}, K. and {Jones}, P.~A. and {Kendrew}, S. and {Mills}, E.~A.~C. and {Molinari}, S. and {Moore}, T.~J.~T. and {Ott}, J. and {Pillai}, T. and {Rathborne}, J. and {Schilke}, P. and {Schmiedeke}, A. and {Testi}, L. and {Walker}, D. and {Walsh}, A. and {Zhang}, Q.},
        title = "{Molecular gas kinematics within the central 250 pc of the Milky Way}",
      journal = {\mnras},
     keywords = {stars: formation, ISM: clouds, ISM: kinematics and dynamics, ISM: structure, Galaxy: centre, galaxies: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = apr,
       volume = {457},
       number = {3},
        pages = {2675-2702},
          doi = {10.1093/mnras/stw121},
archivePrefix = {arXiv},
       eprint = {1601.03732},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.457.2675H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2019MNRAS.485.2457H,
       author = {{Henshaw}, J.~D. and {Ginsburg}, A. and {Haworth}, T.~J. and {Longmore}, S.~N. and {Kruijssen}, J.~M.~D. and {Mills}, E.~A.~C. and {Sokolov}, V. and {Walker}, D.~L. and {Barnes}, A.~T. and {Contreras}, Y. and {Bally}, J. and {Battersby}, C. and {Beuther}, H. and {Butterfield}, N. and {Dale}, J.~E. and {Henning}, T. and {Jackson}, J.~M. and {Kauffmann}, J. and {Pillai}, T. and {Ragan}, S. and {Riener}, M. and {Zhang}, Q.},
        title = "{`The Brick' is not a brick: a comprehensive study of the structure and dynamics of the central molecular zone cloud G0.253+0.016}",
      journal = {\mnras},
     keywords = {turbulence, stars: formation, ISM: clouds, ISM: kinematics and dynamics, ISM: structure, galaxy: centre, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = may,
       volume = {485},
       number = {2},
        pages = {2457-2485},
          doi = {10.1093/mnras/stz471},
archivePrefix = {arXiv},
       eprint = {1902.02793},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.485.2457H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1972ApJ...175L.127S,
       author = {{Scoville}, N.~Z.},
        title = "{Kinematics of Molecular Clouds Near the Galactic Center}",
      journal = {ApJL},
         year = 1972,
        month = aug,
       volume = {175},
        pages = {L127},
          doi = {10.1086/181000},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1972ApJ...175L.127S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2019PASJ...71S..19T,
       author = {{Tokuyama}, Sekito and {Oka}, Tomoharu and {Takekawa}, Shunya and {Iwata}, Yuhei and {Tsujimoto}, Shiho and {Yamada}, Masaya and {Furusawa}, Maiko and {Nomura}, Mariko},
        title = "{High-resolution CO images of the Galactic central molecular zone}",
      journal = {PASJ},
     keywords = {Galaxy: center, Galaxy: kinematics and dynamics, ISM: molecules, surveys},
         year = 2019,
        month = dec,
       volume = {71},
          eid = {S19},
        pages = {S19},
          doi = {10.1093/pasj/psy150},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PASJ...71S..19T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2000ApJ...539..273C,
       author = {{Cho}, Jungyeon and {Vishniac}, Ethan T.},
        title = "{The Anisotropy of Magnetohydrodynamic Alfv{\'e}nic Turbulence}",
      journal = {\apj},
     keywords = {ISM: General, Magnetic Fields, Magnetohydrodynamics: MHD, Turbulence, Astrophysics},
         year = 2000,
        month = aug,
       volume = {539},
       number = {1},
        pages = {273-282},
          doi = {10.1086/309213},
archivePrefix = {arXiv},
       eprint = {astro-ph/0003403},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...539..273C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{GL17,
       author = {{Gonz{\'a}lez-Casanova}, Diego F. and {Lazarian}, A.},
        title = "{Velocity Gradients as a Tracer for Magnetic Fields}",
      journal = {\apj},
     keywords = {ISM: kinematics and dynamics, ISM: magnetic fields, magnetohydrodynamics: MHD, turbulence, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jan,
       volume = {835},
       number = {1},
          eid = {41},
        pages = {41},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...835...41G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020A&A...641A..12P,
       author = {{Planck Collaboration} and {Aghanim}, N. and {Akrami}, Y. and {Alves}, M.~I.~R. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Ballardini}, M. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and {Basak}, S. and {Benabed}, K. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bracco}, A. and {Bucher}, M. and {Burigana}, C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Carron}, J. and {Chary}, R. -R. and {Chiang}, H.~C. and {Colombo}, L.~P.~L. and {Combet}, C. and {Crill}, B.~P. and {Cuttaia}, F. and {de Bernardis}, P. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {Di Valentino}, E. and {Dickinson}, C. and {Diego}, J.~M. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dupac}, X. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Falgarone}, E. and {Fantaye}, Y. and {Fernandez-Cobos}, R. and {Ferri{\`e}re}, K. and {Finelli}, F. and {Forastieri}, F. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frolov}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {G{\'e}nova-Santos}, R.~T. and {Gerbino}, M. and {Ghosh}, T. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Green}, G. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Guillet}, V. and {Handley}, W. and {Hansen}, F.~K. and {Helou}, G. and {Herranz}, D. and {Hivon}, E. and {Huang}, Z. and {Jaffe}, A.~H. and {Jones}, W.~C. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kiiveri}, K. and {Kim}, J. and {Krachmalnicoff}, N. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Le Jeune}, M. and {Levrier}, F. and {Liguori}, M. and {Lilje}, P.~B. and {Lindholm}, V. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Ma}, Y. -Z. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Marcos-Caballero}, A. and {Maris}, M. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Matarrese}, S. and {Mauri}, N. and {McEwen}, J.~D. and {Melchiorri}, A. and {Mennella}, A. and {Migliaccio}, M. and {Miville-Desch{\^e}nes}, M. -A. and {Molinari}, D. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Moss}, A. and {Natoli}, P. and {Pagano}, L. and {Paoletti}, D. and {Patanchon}, G. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Polastri}, L. and {Polenta}, G. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reinecke}, M. and {Remazeilles}, M. and {Renzi}, A. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Ruiz-Granados}, B. and {Salvati}, L. and {Sandri}, M. and {Savelainen}, M. and {Scott}, D. and {Sirignano}, C. and {Sunyaev}, R. and {Suur-Uski}, A. -S. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Tenti}, M. and {Toffolatti}, L. and {Tomasi}, M. and {Trombetti}, T. and {Valiviita}, J. and {Vansyngel}, F. and {Van Tent}, B. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wandelt}, B.~D. and {Wehus}, I.~K. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck 2018 results. XII. Galactic astrophysics using polarized dust emission}",
      journal = {\aap},
     keywords = {polarization, magnetic fields, turbulence, dust, extinction, local insterstellar matter, submillimeter: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = sep,
       volume = {641},
          eid = {A12},
        pages = {A12},
          doi = {10.1051/0004-6361/201833885},
archivePrefix = {arXiv},
       eprint = {1807.06212},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...641A..12P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{YL17a,
       author = {{Yuen}, Ka Ho and {Lazarian}, A.},
        title = "{Tracing Interstellar Magnetic Field Using Velocity Gradient Technique: Application to Atomic Hydrogen Data}",
      journal = {\apjl},
     keywords = {ISM: general, ISM: magnetic fields, ISM: structure, magnetohydrodynamics: MHD, radio lines: ISM, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2017,
        month = mar,
       volume = {837},
       number = {2},
          eid = {L24},
        pages = {L24},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...837L..24Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...537..720L,
       author = {{Lazarian}, A. and {Pogosyan}, D.},
        title = "{Velocity Modification of H I Power Spectrum}",
      journal = {\apj},
     keywords = {Galaxy: Structure, ISM: Kinematics and Dynamics, Radio Lines: ISM, Astrophysics},
         year = 2000,
        month = jul,
       volume = {537},
       number = {2},
        pages = {720-748},
          doi = {10.1086/309040},
archivePrefix = {arXiv},
       eprint = {astro-ph/9901241},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...537..720L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CMZ,
       author = {{Hu}, Yue and {Lazarian}, A. and {Wang}, Q. Daniel},
        title = "{Multi-scale Magnetic Fields in the Central Molecular Zone: Inference from the Gradient Technique}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = may,
          eid = {arXiv:2105.03605},
        pages = {arXiv:2105.03605},
archivePrefix = {arXiv},
       eprint = {2105.03605},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210503605H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{H2,
       author = {{Hu}, Yue and {Lazarian}, A. and {Bialy}, Shmuel},
        title = "{Study Turbulence and Probe Magnetic Fields Using the Gradient Technique: Application to H I-to-H$_{2}$ Transition Regions}",
      journal = {\apj},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, 847, 845, 839, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = dec,
       volume = {905},
       number = {2},
          eid = {129},
        pages = {129},
          doi = {10.3847/1538-4357/abc3c6},
archivePrefix = {arXiv},
       eprint = {2008.00387},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...905..129H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014MNRAS.440.3370K,
       author = {{Kruijssen}, J.~M. Diederik and {Longmore}, Steven N. and {Elmegreen}, Bruce G. and {Murray}, Norman and {Bally}, John and {Testi}, Leonardo and {Kennicutt}, Robert C.},
        title = "{What controls star formation in the central 500 pc of the Galaxy?}",
      journal = {\mnras},
     keywords = {stars: formation, Galaxy: centre, galaxies: evolution, galaxies: ISM, galaxies: starburst, galaxies: star formation, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = jun,
       volume = {440},
       number = {4},
        pages = {3370-3391},
          doi = {10.1093/mnras/stu494},
archivePrefix = {arXiv},
       eprint = {1303.6286},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.440.3370K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013MNRAS.429..987L,
       author = {{Longmore}, S.~N. and {Bally}, J. and {Testi}, L. and {Purcell}, C.~R. and {Walsh}, A.~J. and {Bressert}, E. and {Pestalozzi}, M. and {Molinari}, S. and {Ott}, J. and {Cortese}, L. and {Battersby}, C. and {Murray}, N. and {Lee}, E. and {Kruijssen}, J.~M.~D. and {Schisano}, E. and {Elia}, D.},
        title = "{Variations in the Galactic star formation rate and density thresholds for star formation}",
      journal = {\mnras},
     keywords = {masers, stars: formation, stars: massive, ISM: clouds, ISM: evolution, Galaxy: centre, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = feb,
       volume = {429},
       number = {2},
        pages = {987-1000},
          doi = {10.1093/mnras/sts376},
archivePrefix = {arXiv},
       eprint = {1208.4256},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.429..987L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2010Natur.463...65C,
       author = {{Crocker}, Roland M. and {Jones}, David I. and {Melia}, Fulvio and {Ott}, J{\"u}rgen and {Protheroe}, Raymond J.},
        title = "{A lower limit of 50 microgauss for the magnetic field near the Galactic Centre}",
      journal = {\nat},
     keywords = {Astrophysics - Galaxy Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2010,
        month = jan,
       volume = {463},
       number = {7277},
        pages = {65-67},
          doi = {10.1038/nature08635},
archivePrefix = {arXiv},
       eprint = {1001.1275},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010Natur.463...65C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017MNRAS.469.2263B,
       author = {{Barnes}, A.~T. and {Longmore}, S.~N. and {Battersby}, C. and {Bally}, J. and {Kruijssen}, J.~M.~D. and {Henshaw}, J.~D. and {Walker}, D.~L.},
        title = "{Star formation rates and efficiencies in the Galactic Centre}",
      journal = {\mnras},
     keywords = {stars: formation, ISM: clouds, H $\lt$sc$\gt$II$\lt$/sc$\gt$ regions, Galaxy: centre, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = aug,
       volume = {469},
       number = {2},
        pages = {2263-2285},
          doi = {10.1093/mnras/stx941},
archivePrefix = {arXiv},
       eprint = {1704.03572},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.469.2263B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...761..156F,
       author = {{Federrath}, Christoph and {Klessen}, Ralf S.},
        title = "{The Star Formation Rate of Turbulent Magnetized Clouds: Comparing Theory, Simulations, and Observations}",
      journal = {\apj},
     keywords = {ISM: clouds, ISM: kinematics and dynamics, ISM: structure, magnetohydrodynamics: MHD, stars: formation, turbulence, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2012,
        month = dec,
       volume = {761},
       number = {2},
          eid = {156},
        pages = {156},
          doi = {10.1088/0004-637X/761/2/156},
archivePrefix = {arXiv},
       eprint = {1209.2856},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...761..156F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014PhR...539...49K,
       author = {{Krumholz}, Mark R.},
        title = "{The big problems in star formation: The star formation rate, stellar clustering, and the initial mass function}",
      journal = {\physrep},
     keywords = {Galaxies: star formation, ISM: clouds, ISM: molecules, Stars: formation, Stars: luminosity function, mass function, Turbulence, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = jun,
       volume = {539},
        pages = {49-134},
          doi = {10.1016/j.physrep.2014.02.001},
archivePrefix = {arXiv},
       eprint = {1402.0867},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014PhR...539...49K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018ApJ...863..118B,
       author = {{Burkhart}, Blakesley},
        title = "{The Star Formation Rate in the Gravoturbulent Interstellar Medium}",
      journal = {\apj},
     keywords = {galaxies: star formation, magnetohydrodynamics: MHD, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = aug,
       volume = {863},
       number = {2},
          eid = {118},
        pages = {118},
          doi = {10.3847/1538-4357/aad002},
archivePrefix = {arXiv},
       eprint = {1801.05428},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...863..118B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hu20,
       author = {{Hu}, Yue and {Lazarian}, A. and {Yuen}, Ka Ho},
        title = "{Velocity Gradient in the Presence of Self-gravity: Identifying Gravity-induced Inflow and Determining Collapsing Stage}",
      journal = {\apj},
     keywords = {845, 1569, 847, 1565, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = jul,
       volume = {897},
       number = {2},
          eid = {123},
        pages = {123},
          doi = {10.3847/1538-4357/ab9948},
archivePrefix = {arXiv},
       eprint = {2002.06754},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...897..123H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1988ApJ...333..729W,
       author = {{Werner}, M.~W. and {Davidson}, J.~A. and {Morris}, M. and {Novak}, G. and {Platt}, S.~R. and {Hildebrand}, R.~H.},
        title = "{The Polarization of the Far-Infrared Radiation from the Galactic Center}",
      journal = {\apj},
     keywords = {Cosmic Dust, Far Infrared Radiation, Galactic Nuclei, Infrared Sources (Astronomy), Linear Polarization, Thermal Emission, H Ii Regions, Interstellar Magnetic Fields, Interstellar Matter, Star Clusters, Astrophysics, GALAXIES: THE GALAXY, GALAXIES: NUCLEI, INFRARED: SOURCES, POLARIZATION},
         year = 1988,
        month = oct,
       volume = {333},
        pages = {729},
          doi = {10.1086/166781},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988ApJ...333..729W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1990IAUS..140..361M,
       author = {{Morris}, Mark},
        title = "{The Magnetic Field in the Inner 70-PARSECS of the Milky-Way}",
     keywords = {Galactic Nuclei, Interstellar Magnetic Fields, Magnetic Field Configurations, Milky Way Galaxy, Molecular Clouds, Radio Frequencies, Ring Currents, Astrophysics},
    booktitle = {Galactic and Intergalactic Magnetic Fields},
         year = 1990,
       editor = {{Beck}, R. and {Kronberg}, P.~P. and {Wielebinski}, R.},
       volume = {140},
        month = jan,
        pages = {361},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1990IAUS..140..361M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...529..241N,
       author = {{Novak}, G. and {Dotson}, J.~L. and {Dowell}, C.~D. and {Hildebrand}, R.~H. and {Renbarger}, T. and {Schleuning}, D.~A.},
        title = "{Submillimeter Polarimetric Observations of the Galactic Center}",
      journal = {\apj},
     keywords = {GALAXY: CENTER, INFRARED: ISM: CONTINUUM, ISM: INDIVIDUAL (SAGITTARIUS A), ISM: MAGNETIC FIELDS, POLARIZATION, Galaxy: Center, Infrared: ISM: Continuum, ISM: individual (Sagittarius A), ISM: Magnetic Fields, Polarization},
         year = 2000,
        month = jan,
       volume = {529},
       number = {1},
        pages = {241-250},
          doi = {10.1086/308231},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...529..241N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005MNRAS.360.1305R,
       author = {{Roy}, Subhashis and {Rao}, A. Pramesh and {Subrahmanyan}, Ravi},
        title = "{Extragalactic sources towards the central region of the Galaxy}",
      journal = {\mnras},
     keywords = {techniques: polarimetric, HII regions, Galaxy: centre, radio continuum: ISM, Astrophysics},
         year = 2005,
        month = jul,
       volume = {360},
       number = {4},
        pages = {1305-1324},
          doi = {10.1111/j.1365-2966.2005.09107.x},
archivePrefix = {arXiv},
       eprint = {0712.0258},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.360.1305R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008A&A...478..435R,
       author = {{Roy}, S. and {Pramesh Rao}, A. and {Subrahmanyan}, R.},
        title = "{Magnetic field near the central region of the Galaxy: rotation measure of extragalactic sources}",
      journal = {\aap},
     keywords = {ISM: magnetic fields, Galaxy: center, techniques: polarimetric, Astrophysics},
         year = 2008,
        month = feb,
       volume = {478},
       number = {2},
        pages = {435-442},
          doi = {10.1051/0004-6361:20066470},
archivePrefix = {arXiv},
       eprint = {0712.0269},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...478..435R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1990ApJ...362..114H,
       author = {{Hildebrand}, R.~H. and {Gonatas}, D.~P. and {Platt}, S.~R. and {Wu}, X.~D. and {Davidson}, J.~A. and {Werner}, M.~W. and {Novak}, G. and {Morris}, M.},
        title = "{The Magnetic Field in the Dust Ring at the Center of the Galaxy}",
      journal = {\apj},
     keywords = {Accretion Disks, Cosmic Dust, Galactic Nuclei, Interstellar Magnetic Fields, Milky Way Galaxy, Ring Structures, Thermal Emission, Angular Momentum, Far Infrared Radiation, Interstellar Matter, Astrophysics, GALAXIES: NUCLEI, GALAXIES: THE GALAXY, INTERSTELLAR: GRAINS, INTERSTELLAR: MAGNETIC FIELDS, POLARIZATION},
         year = 1990,
        month = oct,
       volume = {362},
        pages = {114},
          doi = {10.1086/169248},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1990ApJ...362..114H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2007SPIE.6678E..0DV,
       author = {{Vaillancourt}, John E. and {Chuss}, David T. and {Crutcher}, Richard M. and {Dotson}, Jessie L. and {Dowell}, C. Darren and {Harper}, D. Al and {Hildebrand}, Roger H. and {Jones}, Terry J. and {Lazarian}, Alexandre and {Novak}, Giles and {Werner}, Michael W.},
        title = "{Far-infrared polarimetry from the Stratospheric Observatory for Infrared Astronomy}",
     keywords = {Astrophysics},
    booktitle = {Infrared Spaceborne Remote Sensing and Instrumentation XV},
         year = 2007,
       editor = {{Strojnik-Scholl}, Marija},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {6678},
        month = sep,
          eid = {66780D},
        pages = {66780D},
          doi = {10.1117/12.730922},
archivePrefix = {arXiv},
       eprint = {0711.3047},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007SPIE.6678E..0DV},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LY18a,
       author = {{Lazarian}, A. and {Yuen}, Ka Ho},
        title = "{Tracing Magnetic Fields with Spectroscopic Channel Maps}",
      journal = {\apj},
     keywords = {ISM: magnetic fields, ISM: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = jan,
       volume = {853},
       number = {1},
          eid = {96},
        pages = {96},
          doi = {10.3847/1538-4357/aaa241},
archivePrefix = {arXiv},
       eprint = {1703.03119},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...853...96L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ARA&A..53..501A,
       author = {{Andersson}, B. -G. and {Lazarian}, A. and {Vaillancourt}, John E.},
        title = "{Interstellar Dust Grain Alignment}",
      journal = {\araa},
         year = 2015,
        month = aug,
       volume = {53},
        pages = {501-539},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ARA&A..53..501A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2007ApJ...669L..77L,
       author = {{Lazarian}, A. and {Hoang}, Thiem},
        title = "{Subsonic Mechanical Alignment of Irregular Grains}",
      journal = {\apjl},
     keywords = {ISM: Dust, Extinction, ISM: Magnetic Fields, Polarization, Astrophysics},
         year = 2007,
        month = nov,
       volume = {669},
       number = {2},
        pages = {L77-L80},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...669L..77L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018JAI.....740008H,
       author = {{Harper}, Doyal A. and {Runyan}, Marcus C. and {Dowell}, C. Darren and {Wirth}, C. Jesse and {Amato}, Michael and {Ames}, Troy and {Amiri}, Mandana and {Banks}, Stuart and {Bartels}, Arlin and {Benford}, Dominic J. and {Berthoud}, Marc and {Buchanan}, Ernest and {Casey}, Sean and {Chapman}, Nicholas L. and {Chuss}, David T. and {Cook}, Brant and {Derro}, Rebecca and {Dotson}, Jessie L. and {Evans}, Rhodri and {Fixsen}, Dale and {Gatley}, Ian and {Guerra}, Jordan A. and {Halpern}, Mark and {Hamilton}, Ryan T. and {Hamlin}, Louise A. and {Hansen}, Christopher J. and {Heimsath}, Stephen and {Hermida}, Alfonso and {Hilton}, Gene C. and {Hirsch}, Robert and {Hollister}, Matthew I. and {Hostetter}, Carl F. and {Irwin}, Kent and {Jhabvala}, Christine A. and {Jhabvala}, Murzban and {Kastner}, Joel and {Kov{\'a}cs}, Attila and {Lin}, Sean and {Loewenstein}, Robert F. and {Looney}, Leslie W. and {Lopez-Rodriguez}, Enrique and {Maher}, Stephen F. and {Michail}, Joseph M. and {Miller}, Timothy M. and {Moseley}, S. Harvey and {Novak}, Giles and {Pernic}, Robert J. and {Rennick}, Timothy and {Rhody}, Harvey and {Sandberg}, Eric and {Sandford}, Dale and {Santos}, Fabio Pereira and {Shafer}, Rick and {Sharp}, Elmer H. and {Shirron}, Peter and {Siah}, Javad and {Silverberg}, Robert and {Sparr}, Leroy M. and {Spotz}, Robert and {Staguhn}, Johannes G. and {Toorian}, Armen S. and {Towey}, Shannon and {Tuttle}, Jim and {Vaillancourt}, John and {Voellmer}, George and {Volpert}, Carolyn G. and {Wang}, Shu-I. and {Wollack}, Edward J.},
        title = "{HAWC+, the Far-Infrared Camera and Polarimeter for SOFIA}",
      journal = {Journal of Astronomical Instrumentation},
     keywords = {Instrumentation, polarimeters, camera, far-infrared, detectors, stars, formation, dust},
         year = 2018,
        month = jan,
       volume = {7},
       number = {4},
          eid = {1840008-1025},
        pages = {1840008-1025},
          doi = {10.1142/S2251171718400081},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018JAI.....740008H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015A&A...576A.104P,
       author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and {Alina}, D. and {Alves}, M.~I.~R. and {Armitage-Caplan}, C. and {Arnaud}, M. and {Arzoumanian}, D. and {Ashdown}, M. and {Atrio-Barandela}, F. and {Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Battaner}, E. and {Benabed}, K. and {Benoit-L{\'e}vy}, A. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bracco}, A. and {Burigana}, C. and {Butler}, R.~C. and {Cardoso}, J. -F. and {Catalano}, A. and {Chamballu}, A. and {Chary}, R. -R. and {Chiang}, H.~C. and {Christensen}, P.~R. and {Colombi}, S. and {Colombo}, L.~P.~L. and {Combet}, C. and {Couchot}, F. and {Coulais}, A. and {Crill}, B.~P. and {Curto}, A. and {Cuttaia}, F. and {Danese}, L. and {Davies}, R.~D. and {Davis}, R.~J. and {de Bernardis}, P. and {de Gouveia Dal Pino}, E.~M. and {de Rosa}, A. and {de Zotti}, G. and {Delabrouille}, J. and {D{\'e}sert}, F. -X. and {Dickinson}, C. and {Diego}, J.~M. and {Donzelli}, S. and {Dor{\'e}}, O. and {Douspis}, M. and {Dunkley}, J. and {Dupac}, X. and {Efstathiou}, G. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Falgarone}, E. and {Ferri{\`e}re}, K. and {Finelli}, F. and {Forni}, O. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Galeotta}, S. and {Ganga}, K. and {Ghosh}, T. and {Giard}, M. and {Giraud-H{\'e}raud}, Y. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gregorio}, A. and {Gruppuso}, A. and {Guillet}, V. and {Hansen}, F.~K. and {Harrison}, D.~L. and {Helou}, G. and {Hern{\'a}ndez-Monteagudo}, C. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Hobson}, M. and {Holmes}, W.~A. and {Hornstrup}, A. and {Huffenberger}, K.~M. and {Jaffe}, A.~H. and {Jaffe}, T.~R. and {Jones}, W.~C. and {Juvela}, M. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kisner}, T.~S. and {Kneissl}, R. and {Knoche}, J. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {L{\"a}hteenm{\"a}ki}, A. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lawrence}, C.~R. and {Leahy}, J.~P. and {Leonardi}, R. and {Levrier}, F. and {Liguori}, M. and {Lilje}, P.~B. and {Linden-V{\o}rnle}, M. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maffei}, B. and {Magalh{\~a}es}, A.~M. and {Maino}, D. and {Mandolesi}, N. and {Maris}, M. and {Marshall}, D.~J. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Matarrese}, S. and {Mazzotta}, P. and {Melchiorri}, A. and {Mendes}, L. and {Mennella}, A. and {Migliaccio}, M. and {Miville-Desch{\^e}nes}, M. -A. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Mortlock}, D. and {Munshi}, D. and {Murphy}, J.~A. and {Naselsky}, P. and {Nati}, F. and {Natoli}, P. and {Netterfield}, C.~B. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {Oxborrow}, C.~A. and {Pagano}, L. and {Pajot}, F. and {Paladini}, R. and {Paoletti}, D. and {Pasian}, F. and {Pearson}, T.~J. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Piacentini}, F. and {Piat}, M. and {Pietrobon}, D. and {Plaszczynski}, S. and {Poidevin}, F. and {Pointecouteau}, E. and {Polenta}, G. and {Popa}, L. and {Pratt}, G.~W. and {Prunet}, S. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reach}, W.~T. and {Rebolo}, R. and {Reinecke}, M. and {Remazeilles}, M. and {Renault}, C. and {Ricciardi}, S. and {Riller}, T. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Rusholme}, B. and {Sandri}, M. and {Savini}, G. and {Scott}, D. and {Spencer}, L.~D. and {Stolyarov}, V. and {Stompor}, R. and {Sudiwala}, R. and {Sutton}, D. and {Suur-Uski}, A. -S. and {Sygnet}, J. -F. and {Tauber}, J.~A. and {Terenzi}, L. and {Toffolatti}, L. and {Tomasi}, M. and {Tristram}, M. and {Tucci}, M. and {Umana}, G. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, B. and {Vielva}, P. and {Villa}, F. and {Wade}, L.~A. and {Wandelt}, B.~D. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck intermediate results. XIX. An overview of the polarized thermal emission from Galactic dust}",
      journal = {\aap},
     keywords = {ISM: general, dust, extinction, ISM: magnetic fields, ISM:, clouds, submillimeter: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = apr,
       volume = {576},
          eid = {A104},
        pages = {A104},
          doi = {10.1051/0004-6361/201424082},
archivePrefix = {arXiv},
       eprint = {1405.0871},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...576A.104P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1986AJ.....92..818T,
       author = {{Tsuboi}, M. and {Inoue}, M. and {Handa}, T. and {Tabara}, H. and {Kato}, T. and {Sofue}, Y. and {Kaifu}, N.},
        title = "{Prominent polarized plumes in the Galactic Center region and their magnetic field.}",
      journal = {\aj},
     keywords = {Galactic Nuclei, Interstellar Magnetic Fields, Linear Polarization, Milky Way Galaxy, Radio Astronomy, Depolarization, Magnetic Field Configurations, Plumes, Polarization Characteristics, Astrophysics},
         year = 1986,
        month = oct,
       volume = {92},
        pages = {818-824},
          doi = {10.1086/114215},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1986AJ.....92..818T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1990IAUS..140..361M,
       author = {{Morris}, Mark},
        title = "{The Magnetic Field in the Inner 70-PARSECS of the Milky-Way}",
     keywords = {Galactic Nuclei, Interstellar Magnetic Fields, Magnetic Field Configurations, Milky Way Galaxy, Molecular Clouds, Radio Frequencies, Ring Currents, Astrophysics},
    booktitle = {Galactic and Intergalactic Magnetic Fields},
         year = 1990,
       editor = {{Beck}, R. and {Kronberg}, P.~P. and {Wielebinski}, R.},
       volume = {140},
        month = jan,
        pages = {361},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1990IAUS..140..361M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999ApJ...521L..41L,
       author = {{Lang}, Cornelia C. and {Anantharamaiah}, K.~R. and {Kassim}, N.~E. and {Lazio}, T.~J.~W.},
        title = "{Discovery of a Nonthermal Galactic Center Filament (G358.85+0.47) Parallel to the Galactic Plane}",
      journal = {\apjl},
     keywords = {GALAXY: CENTER, ISM: MAGNETIC FIELDS, RADIO CONTINUUM: ISM, Galaxy: Center, ISM: Magnetic Fields, Radio Continuum: ISM, Astrophysics},
         year = 1999,
        month = aug,
       volume = {521},
       number = {1},
        pages = {L41-L44},
          doi = {10.1086/312180},
archivePrefix = {arXiv},
       eprint = {astro-ph/9906285},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...521L..41L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019ApJ...884..170P,
       author = {{Par{\'e}}, Dylan M. and {Lang}, Cornelia C. and {Morris}, Mark R. and {Moore}, Hailey and {Mao}, Sui Ann},
        title = "{A VLA Polarimetric Study of the Galactic Center Radio Arc: Characterizing Polarization, Rotation Measure, and Magnetic Field Properties}",
      journal = {\apj},
     keywords = {Galactic center, Galaxy magnetic fields, Milky Way magnetic fields, Interstellar synchrotron emission, Radio astronomy, Very Large Array, Radio continuum emission, Non-thermal radiation sources, 565, 604, 1057, 856, 1338, 1766, 1340, 1119, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = oct,
       volume = {884},
       number = {2},
          eid = {170},
        pages = {170},
          doi = {10.3847/1538-4357/ab45ed},
archivePrefix = {arXiv},
       eprint = {1909.08268},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...884..170P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PCA,
       author = {{Hu}, Yue and {Yuen}, Ka Ho and {Lazarian}, A.},
        title = "{Improving the accuracy of magnetic field tracing by velocity gradients: principal component analysis}",
      journal = {\mnras},
     keywords = {magnetohydrodynamics (MHD), turbulence, methods: numerical, ISM: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = oct,
       volume = {480},
       number = {1},
        pages = {1333-1339},
          doi = {10.1093/mnras/sty1807},
archivePrefix = {arXiv},
       eprint = {1802.08772},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.480.1333H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GS95,
       author = {{Goldreich}, P. and {Sridhar}, S.},
        title = "{Toward a Theory of Interstellar Turbulence. II. Strong Alfvenic Turbulence}",
      journal = {\apj},
     keywords = {Interstellar Space, Magnetic Fields, Magnetohydrodynamic Turbulence, Magnetohydrodynamic Waves, Electron Density (Concentration), Energy Spectra, Radio Waves, Variations, Wave Scattering, Astrophysics, ISM: GENERAL, MAGNETOHYDRODYNAMICS: MHD, TURBULENCE},
         year = 1995,
        month = jan,
       volume = {438},
        pages = {763},
          doi = {10.1086/175121},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...438..763G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LV99,
       author = {{Lazarian}, A. and {Vishniac}, Ethan T.},
        title = "{Reconnection in a Weakly Stochastic Field}",
      journal = {\apj},
     keywords = {GALAXIES: MAGNETIC FIELDS, MAGNETOHYDRODYNAMICS: MHD, Galaxies: Magnetic Fields, Magnetohydrodynamics: MHD, Astrophysics, Physics - Fluid Dynamics, Physics - Geophysics, Physics - Plasma Physics, Physics - Space Physics},
         year = 1999,
        month = jun,
       volume = {517},
       number = {2},
        pages = {700-718},
          doi = {10.1086/307233},
archivePrefix = {arXiv},
       eprint = {astro-ph/9811037},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...517..700L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2021ApJ...911...37H,
       author = {{Hu}, Yue and {Xu}, Siyao and {Lazarian}, A.},
        title = "{Anisotropies in Compressible MHD Turbulence: Probing Magnetic Fields and Measuring Magnetization}",
      journal = {\apj},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, 847, 845, 839, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = apr,
       volume = {911},
       number = {1},
          eid = {37},
        pages = {37},
          doi = {10.3847/1538-4357/abea18},
archivePrefix = {arXiv},
       eprint = {2012.06039},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...911...37H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018arXiv180200024Y,
       author = {{Yuen}, Ka Ho and {Lazarian}, A.},
        title = "{Advancing the Velocity Gradient Technique: Using Gradient Amplitudes and handling thermal broadening}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jan,
          eid = {arXiv:1802.00024},
        pages = {arXiv:1802.00024},
archivePrefix = {arXiv},
       eprint = {1802.00024},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv180200024Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...740..117E,
       author = {{Esquivel}, A. and {Lazarian}, A.},
        title = "{Velocity Anisotropy as a Diagnostic of the Magnetization of the Interstellar Medium and Molecular Clouds}",
      journal = {\apj},
     keywords = {ISM: general, ISM: structure, magnetohydrodynamics: MHD, radio lines: ISM, turbulence, Astrophysics - Astrophysics of Galaxies},
         year = 2011,
        month = oct,
       volume = {740},
       number = {2},
          eid = {117},
        pages = {117},
          doi = {10.1088/0004-637X/740/2/117},
archivePrefix = {arXiv},
       eprint = {1108.0693},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...740..117E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021ApJ...910...88X,
       author = {{Xu}, Siyao and {Hu}, Yue},
        title = "{Measuring Magnetization with Rotation Measures and Velocity Centroids in Supersonic MHD Turbulence}",
      journal = {\apj},
     keywords = {Interstellar medium, Magnetohydrodynamics, Interstellar magnetic fields, 847, 1964, 845, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = apr,
       volume = {910},
       number = {2},
          eid = {88},
        pages = {88},
          doi = {10.3847/1538-4357/abe403},
archivePrefix = {arXiv},
       eprint = {2102.05647},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...910...88X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021ApJ...915...67H,
       author = {{Hu}, Yue and {Lazarian}, A. and {Xu}, Siyao},
        title = "{Anisotropic Turbulence in Position-Position-Velocity Space: Probing Three-dimensional Magnetic Fields}",
      journal = {\apj},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, 847, 845, 839, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = jul,
       volume = {915},
       number = {1},
          eid = {67},
        pages = {67},
          doi = {10.3847/1538-4357/ac00ab},
archivePrefix = {arXiv},
       eprint = {2104.02842},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...915...67H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Liu21,
       author = {{Liu}, Mingrui and {Hu}, Yue and {Lazarian}, Alex},
        title = "{Velocity Gradients: Magnetic Field Tomography towards the Supernova Remnant W44}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = sep,
          eid = {arXiv:2109.13670},
        pages = {arXiv:2109.13670},
archivePrefix = {arXiv},
       eprint = {2109.13670},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210913670L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019A&A...630A..74M,
       author = {{Mangilli}, A. and {Aumont}, J. and {Bernard}, J. -Ph. and {Buzzelli}, A. and {de Gasperis}, G. and {Durrive}, J.~B. and {Ferriere}, K. and {Fo{\"e}nard}, G. and {Hughes}, A. and {Lacourt}, A. and {Misawa}, R. and {Montier}, L. and {Mot}, B. and {Ristorcelli}, I. and {Roussel}, H. and {Ade}, P. and {Alina}, D. and {de Bernardis}, P. and {de Gouveia Dal Pino}, E. and {Dubois}, J.~P. and {Engel}, C. and {Guillet}, V. and {Hargrave}, P. and {Laureijs}, R. and {Longval}, Y. and {Maffei}, B. and {Magalhaes}, A.~M. and {Marty}, C. and {Masi}, S. and {Montel}, J. and {Pajot}, F. and {P{\'e}rot}, E. and {Rodriguez}, L. and {Salatino}, M. and {Saccoccio}, M. and {Savini}, G. and {Stever}, S. and {Tauber}, J. and {Tibbs}, C. and {Tucker}, C.},
        title = "{The geometry of the magnetic field in the central molecular zone measured by PILOT}",
      journal = {\aap},
     keywords = {Galaxy: center, polarization, magnetic fields, balloons, methods: data analysis, dust, extinction, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = oct,
       volume = {630},
          eid = {A74},
        pages = {A74},
          doi = {10.1051/0004-6361/201935072},
archivePrefix = {arXiv},
       eprint = {1901.06196},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...630A..74M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2009A&A...505.1183F,
       author = {{Ferri{\`e}re}, K.},
        title = "{Interstellar magnetic fields in the Galactic center region}",
      journal = {\aap},
     keywords = {ISM: magnetic fields, ISM: general, ISM: structure, cosmic rays, Galaxy: center, galaxies: magnetic fields, Astrophysics - Astrophysics of Galaxies},
         year = 2009,
        month = oct,
       volume = {505},
       number = {3},
        pages = {1183-1198},
          doi = {10.1051/0004-6361/200912617},
archivePrefix = {arXiv},
       eprint = {0908.2037},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&A...505.1183F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1999ASPC..186..519S,
       author = {{Sofue}, Y. and {Lang}, C.~C.},
        title = "{The Magnetic Field in the Galactic Center}",
    booktitle = {The Central Parsecs of the Galaxy},
         year = 1999,
       editor = {{Falcke}, Heino and {Cotera}, Angela and {Duschl}, Wolfgang J. and {Melia}, Fulvio and {Rieke}, Marcia J.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {186},
        month = jun,
        pages = {519},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ASPC..186..519S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


